Are More LLM Calls All You Need? Towards Scaling Laws of Compound Inference Systems

Many recent state-of-the-art results in language tasks were achieved using compound systems that perform multiple Language Model (LM) calls and aggregate their responses. However, there is little understanding of how the number of LM calls - e.g., when asking the LM to answer each question multiple times and taking a majority vote - affects such a compound system's performance. In this paper, we initiate the study of scaling properties of compound inference systems. We analyze, theoretically and empirically, how the number of LM calls affects the performance of Vote and Filter-Vote, two of the simplest compound system designs, which aggregate LM responses via majority voting, optionally applying LM filters. We find, surprisingly, that across multiple language tasks, the performance of both Vote and Filter-Vote can first increase but then decrease as a function of the number of LM calls. Our theoretical results suggest that this non-monotonicity is due to the diversity of query difficulties within a task: more LM calls lead to higher performance on "easy" queries, but lower performance on "hard" queries, and non-monotone behavior can emerge when a task contains both types of queries. This insight then allows us to compute, from a small number of samples, the number of LM calls that maximizes system performance, and define an analytical scaling model for both systems. Experiments show that our scaling model can accurately predict the performance of Vote and Filter-Vote systems and thus find the optimal number of LM calls to make.

==> experiment_backup.tex <==

\section{Additional Analysis}

dichotomy on the effects of the generator numbers on the pairwise selector

Let $M$ be the comparison matrix. 
Each pairwise comparison is a noisy estimation of $M$.

$\tau_i(M) = \sum^{}_{j}M_{ij}$ is the score for the $i$'s unique generation.

$\hat{i} = \arg \max \tau_i(M)$.

The dichotomy: 

If $\hat{i}=i^*$, then more generations improve the selector's quality.

Otherwise, more generations can only be harmful.

----------TODO--------
RQ1: How to formally model the selector? 

A: A selector $S$ takes one query $q$ and $K$ candidate answers 
 $a_1, a_2, \cdots, a_K$ as input, and then returns one of the answers. To avoid using random functions, we use $\delta$ to denote the randomness of the model selector.

 $a_S = S(q,a_1,a_2,\cdots. a_K, \delta)$.

 How do we understand the quality of the above selector? 

The 

------TODO-------

RQ1. What are ways to aggregate the candidate answers beyond the majority vote? 


RQ2. How do we analyze the performance? 

RQ3. How can we validate the observations?

Answer to RQ1: We should separate two concepts: (i) generation difficulty, i.e., whether the majority answer is correct, and (ii) judgment difficulty, i.e., whether an LLM can find the correct answer.

Answer to RQ2: 

Given a query, $q$, 

$a_1, a_2, ...,a_n$.


Answer to RQ3: 




Consider a 


Another key insight:


\section{Additional Experiments}

We study three different aggregation functions, namely, majority vote, llm judge, and pairwise judgment. 

\paragraph{Accuracy.}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/selector/abstract_algebra_gpt4_overall.png}
         \caption{All queries}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/selector/abstract_algebra_gpt4_easy.png}
         \caption{Easy queries}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/selector/abstract_algebra_gpt4_hard.png}
         \caption{Hard queries}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Performance of \LLMNets{} with different selectors on abstract algebra. All generators and selectors are GPT-4-0125-preview. All experiments were averaged over three runs.  A few points: 1. There seems to be a u-shape for the LLM judge as the selector. 2. Pairwise comparison seems to work much better than other two selectors on the hard queries, but becomes worse on the easy queries. 3. Next steps: Predict which selector is better. This is highly related to the difficulty prediction problem.}
        \label{fig:three graphs}
\end{figure}

\paragraph{Performance breakdown.}


\subsection{}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/collegemath_judge.png}
    \caption{Different aggregation strategies on MMLU College Math. Overall, we can see that the judge systems offer a significant performance gain.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/businessethics_judge.png}
    \caption{Different aggregation strategies on MMLU business ethics. Overall, we can see that the majority voting systems offer a significant performance gain.}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/abstractalgebra_judge.png}
    \caption{Different aggregation strategies on MMLU abstract algebra. Overall, we can see that  majority voting systems and judge systems are on par.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/realworld/gpqa_gpqa_diamond_gpt-3.5-turbo-0125_aggregate_0_0_1000_full.pdf}
         \caption{Full}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/realworld/gpqa_gpqa_diamond_gpt-3.5-turbo-0125_aggregate_0_0_1000_easy.pdf}
         \caption{Easy}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/realworld/gpqa_gpqa_diamond_gpt-3.5-turbo-0125_aggregate_0_0_1000_hard.pdf}
         \caption{Hard}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Performance eval on GPQA diomand. }
        \label{fig:three graphs}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/gpqa_01.png}
    \caption{GPQA difficult transition from 0 enhance to 1 enhance layer.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/gpqa_12.png}
    \caption{GPQA difficult transition from 1 enhance to 2 enhance layer.}
    \label{fig:enter-label}
\end{figure}


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/realworld/livecodebench_execution_gpt-3.5-turbo-0125_aggregate_0_0_100_full.pdf}
         \caption{Full}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/realworld/livecodebench_execution_gpt-3.5-turbo-0125_aggregate_0_0_100_easy.pdf}
         \caption{Easy}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/realworld/livecodebench_execution_gpt-3.5-turbo-0125_aggregate_0_0_100_hard.pdf}
         \caption{Hard}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Performance eval on LivecodeBench  (execution).  \texttt{\char96\char96\char96}
}
        \label{fig:three graphs}
\end{figure}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/usmle_Step2_gpt-3.5-turbo-0125_aggregate_1_2_1_full.pdf}
    \caption{USMLE Step 2 Full.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/usmle_Step2_gpt-3.5-turbo-0125_aggregate_1_2_1_easy.pdf}
    \caption{USMLE Step 2 easy.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/usmle_Step2_gpt-3.5-turbo-0125_aggregate_1_2_1_hard.pdf}
    \caption{USMLE Step 2 difficult.}
    \label{fig:enter-label}
\end{figure}

Breakdown performance on hard and easy queries

Randomized answer order fed to the judge


Give the candidate answers without the reasoning steps

More architectures (pairwise, tell the judge what the majority vote is and suggest if change is needed. )

Give the freedom of the judge to generate a new answer

Ask the judge explicitly to do a step-by-step reasoning. 

Contrast approach:
Explictly ask the model to give incorrect answer which sounds correct and then ask the judge to make selection decision based on this info. 

Later on could also do fine-tuning based on this idea.




Some new experiments.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/livecodebench_test.jpg}
    \caption{Livecodebench.}
    \label{fig:enter-label}
\end{figure}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/votingflitering.png}
    \caption{KSP Voting vs Filtering.}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/gpqa_gpqa_diamond_gpt-4-0125-preview_aggregate_0_0_401_False_single_step_scalelaw.pdf}
    \caption{GPQA.}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/realworld/mmlu_collegemath_gpt35.png}
    \caption{MMLU GPT-3.5-turbo.}
    \label{fig:enter-label}
\end{figure}

TODO: experiments with perfect judge. Simulate it via MMLU or find a task with easy judge (e.g., code generations, or words starting with letters, or containing certain words, etc)

TODO: get some examples for the easy/difficulty transfer matrix. When and why a query becomes easier/harder?


What is the takeaway message? Should we use enhance (since the benefit is limited)?

Scientific vs Engineering 


How about some programming problems?


\url{https://github.com/lizhouf/NPHardEval4V/tree/main/Data/SPP/Images}


\section{Analysis on the Filtering approach}

\paragraph{How to model the filtering approach.}
For any fixed query $x$, we quantify the performance of a filter by (i) the probability that an answer is kept given that it is sampled from the correct answer set, denoted by $\alpha$, and (ii) the probability that an answer is kept given that it is sampled from the incorrect answer set, denoted by $\beta$. 
More formally, 

\begin{equation*}
    \alpha=\Pr[z \in h(z) |z  \textit{ is correct}]
\end{equation*}
and 
\begin{equation*}
    \beta=\Pr[z \in h(z) |z  \textit{ is incorrect}]
\end{equation*}


\paragraph{When the filtering approach is better than voting?}
\begin{theorem}
    The filtering approach is better than the voting approach if and only if $\alpha>\beta$.
\end{theorem}



 A key research question to ask is, when is the filter





 \subsection{Scaling Properties on Real-world Datasets}
\begin{figure}[t]
    \centering
    \vspace{0mm}\includegraphics[width=0.90\textwidth]{figure/realworld/InferNetScaleLaws_RealWorld.pdf}
    \caption{\LLMNet{}'s performance and our prediction on real-world datasets. The orange dots are the empirical performance of a one-layer Voting \LLMNet{} averaged over 1000 runs, and the blue lines correspond to the performance predicted by our scaling law. GPT-3.5-turbo-0125 is the LLM adopted by the one-layer Voting \LLMNet{}. Overall, we observe that increasing the number of calls does not always lead to performance gains. This is because its effects are opposite on the easy and hard queries. Our analytical model can accurately predict the performance and thus enables optimal ensemble size selection without an exhaustive search of all possible numbers of calls.   }
    \label{fig:ScaleLaw:RealWorld}
\end{figure}
Finally, we validate the effectiveness of our scaling law on real-world datasets. We focus on three datasets as a first step: college mathematics, business ethics, and college chemistry, curated from the MMLU benchmark~\cite{hendrycks2020measuring}. Each query in these datasets is a multiple-choice question. We use GPT-3.5 to generate candidate answers. For each generation, we add 1 to 2 few-shot examples randomly chosen from a pool of 5 examples to the prompt to encourage diversity. We set the temperature to be 0.7. Here,  a query item is considered easy if the majority vote of 1,000 GPT-3.5's generations is correct, and is considered difficult otherwise. To fit our scaling law, we use the performance evaluated with $1,10,100$ and $1000$ LLM calls as the training data, and then use the estimated scaling law to predict the performance for all other numbers of LLM calls.

Figure \ref{fig:ScaleLaw:RealWorld} shows the overall performance of one-layer Voting \LLMNet{} with varying numbers of LLM calls and also the performance predicted by our scaling law. There are several interesting observations. First, the overall performance is not always monotonically increasing as the number of LLM calls grows. On college mathematics and business ethics, for example,  the performance is maximized at a specific number of LLM calls and becomes worse when the number of LLM calls becomes further away from this unique nubmer. Second, we observe that this counter-intuitive phenomenon can be explained by the performance breakdown on easy and hard subsets. 
In fact, on the easy subsets, the Voting \LLMNet{}'s performance monotonically increases as the more LLM calls are invoked. 
On the other hand, on the hard queries, the performance continuously decays as more LLM calls are invoked. This is also true even if the overall performance is monotone. 
For example, on the college chemistry dataset, increasing the number of LLM calls leads to a continuously improved overall performance, but also a continuously decreasing performance on the hard queries. This reveals a fundamental tradeoff: the number of LLM calls has opposite effects on easy and hard queries, and changing it balances performance on easy and hard queries. Furthermore, our scaling law can accurately predict the performance of Voting \LLMNet{}, on the full data, easy subset, and the hard subset. In practice, this makes it much easier to identify the optimal number of LLM calls: one can simply choose the number that maximizes the predicted performance. 

\subsection{Predicting Query Difficulty}
\begin{table}[t]
  \centering
  \small
  \caption{Zero-shot Difficulty Prediction Performance on real-world datasets. Overall, zero-shot GPT-4-turbo correctly recognizes the difficulty for a large range of queries, although there is still a large room for improvement. %\james{Explain what is blue and orange.}
  }
    %\small
    \begin{tabular}{||c|c|c|c||}
    \hline
    LLM Predictor &
      College Mathematics &
      Business  Ethics &
      College Chemistry
      \bigstrut\\
    \hline
    \hline
    GPT-4 &
      65.7\% &
      67.6\% &
      71.7\%
      \bigstrut\\
    \hline
    GPT-3.5 &
      58.6\% &
      55.5\% &
      51.5\%
      \bigstrut\\
    \hline
    Dummy &
      57.6\% &
      64.6\% &
      60.6\%
      \bigstrut\\
    \hline
    \end{tabular}%
  \label{tab:ScaleLaw:DifficultyPrediction}%
\end{table}%




We also explore how accurately LLMs can infer the item difficulty. In a nutshell, we give an LLM a question item, the response by an \LLMNet{}, and asks the LLM whether the question is difficult to the \LLMNet{}. As a first step, we use GPT-4 and GPT-3.5 as the difficulty predictor, and evaluate their performance as shown in Table \ref{tab:ScaleLaw:DifficultyPrediction}. Interestingly, GPT-3.5 performs poorly as its accuracy is on par with the dummy predictor, which gives the most frequent label (e.g., always ``easy''). On the other hand, GPT-4 seems to predict the item difficulty reasonably well, with 3\% to 11\% improvement compared with the dummy predictor that always predicts the more common class.  

Note that a high-quality difficulty predictor are practically valuable. For example, we can integrate it into a \LLMNet{} to enable fine-grained network size selection. If the query is predicted to be easy, use a large number of LLM calls. Otherwise, only call an LLM a few times. We leave designing high-quanlity difficulty predictors and principled ways to leverage the predictors as future work. % be of practical values. There are other problems e.g., you ask an LLM to guess the password, code generations, etc.. AlphaCode 2, etc.


%TODO: Suppose we have a oracle predictor, how much performance improvement we can get?


\begin{wrapfigure}{r}{0.55\textwidth}
  \begin{center}
    \includegraphics[width=0.45\textwidth]{figure/intro/intro_example.pdf}
  \end{center}
  \caption{The impact of the number of GPT-3.5 calls on performance of \VISFull{} and \FVISFull{} for the MMLU PHYSICS dataset~\cite{hendrycks2020measuring}. We observe a non-monotone trend, e.g., at first, increasing the number of LM calls improves the accuracy of \VISFull{}, but later, it reduces it.}\label{fig:ScaleLaw:intro1}
\end{wrapfigure}

==> macro.tex <==
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{wrapfig}
\usepackage{bbm}
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables
\usepackage{amsthm,amsmath,amssymb}
%\usepackage{graphicx,xspace,verbatim,comment}
%\usepackage{array,color,multirow}
%\usepackage{balance,float,url,amsfonts,alltt}
\usepackage{float,url,amsfonts,alltt}
\usepackage{mathtools,rotating}
\usepackage{ifpdf,fancyvrb}
\usepackage{enumitem}
%\usepackage{algorithm,algpseudocode}
%\usepackage{etoolbox,listings,subcaption}
%\usepackage{bigstrut,morefloats}
%\usepackage[boxruled]{algorithm2e}
%\usepackage{pbox}
%\usepackage{thm-restate}
%\usepackage{todonotes}
%\usepackage[boxruled]{algorithm2e}
%\usepackage{pbox}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{booktabs} % for professional tables
\usepackage{hyperref}

\usepackage{graphicx,xspace,verbatim,comment}
\usepackage{hyperref,array,color,balance,multirow}
\usepackage{balance,float,url,amsfonts,alltt}
\usepackage{mathtools,rotating,amsmath,amssymb}
\usepackage{color,ifpdf,fancyvrb,array}
% \usepackage{algorithm,algpseudocode}
\usepackage{etoolbox,listings}
%\usepackage{subcaption}
\usepackage{bigstrut,morefloats}

%\usepackage[boxruled]{algorithm2e}
\usepackage{pbox}
%\usepackage{natbib}
%\usepackage[boxruled,algo2e]{algorithm2e}
%\usepackage{algorithm}
\usepackage{algpseudocode}

\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}
\newcommand{\eat}[1]{}

\newcommand{\gaussian}[2]{\mathcal{N}(#1,#2)}


\newcommand{\sgn}{\operatorname{sign}}
\newcommand{\indi}{\mathds{1}}
\newcommand{\ie}{{\emph i.e.,} }
\newcommand{\eg}{{\it e.g.}, }
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\C}{\mathbb{C}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\var}{\operatorname{Var}}
\newcommand{\card}{\operatorname{card}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\cov}{\operatorname{Cov}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\vecw}{\mathbf{w}}
\newcommand{\vecwb}{\mathbf{w}}
\newcommand{\tvecw}{\widetilde{\mathbf{w}}}
\newcommand{\tvecwb}{\widetilde{\mathbf{w}}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\ovecv}{\overline{\mathbf{v}}}
\newcommand{\vecy}{\mathbf{y}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\veca}{\mathbf{a}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\vecn}{\mathbf{n}}
\newcommand{\vece}{\mathbf{e}}
\newcommand{\vecz}{\mathbf{z}}
\newcommand{\tvecz}{\widetilde{\mathbf{z}}}
\newcommand{\matA}{\mathbf{A}}
\newcommand{\matP}{\mathbf{P}}
\newcommand{\matD}{\mathbf{D}}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\gradf}{\nabla f}
\newcommand{\tf}{\widetilde{f}}
\newcommand{\gradtf}{\nabla \widetilde{f}}
\newcommand{\gradF}{\nabla F}
\newcommand{\HW}{\textsc{Hogwild!}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\matS}{\mathbf{S}}
\newcommand{\const}{\mathcal{O}(1)}
\newcommand{\bigo}{\mathcal{O}}
\newcommand{\setI}{\mathcal{I}}
\newcommand{\CM}{\textsc{KroMagnon}}
\newcommand{\cdeg}{\overline{\Delta}}
\newcommand{\ct}{\mathcal{O}(1)}
\newcommand{\W}{\mathcal{W}}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\norms}[1]{\|#1\|}
\newcommand{\twonm}[1]{\left\|#1\right\|_2}
\newcommand{\twonms}[1]{\|#1\|_2}
\newcommand{\onenm}[1]{\left\|#1\right\|_1}
\newcommand{\onenms}[1]{\|#1\|_1}
\newcommand{\fbnorm}[1]{\left\|#1\right\|_F}
\newcommand{\fbnorms}[1]{\|#1\|_F}
\newcommand{\prob}[1]{\mathbb{P}\left\{#1\right\}}
\newcommand{\probs}[1]{\mathbb{P}\{#1\}}
\newcommand{\EXP}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\EE}{\ensuremath{\mathbb{E}}}
\newcommand{\EXPS}[1]{\mathbb{E}[#1]}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\innerp}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\innerps}[2]{\langle#1,#2\rangle}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\abss}[1]{|#1|}
\newcommand{\tsp}{^{\rm T}}
\newcommand{\floor}[1]{\lfloor#1\rfloor}
\newcommand{\mt}{B\floor{t/B}}
%\newcommand{\G}{\overline{G}}
%\newcommand{\B}{\overline{B}}
\numberwithin{equation}{section}
\newcommand{\eq}[1]{(\ref{eq:#1})}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\red}[1]{{\color{red}{#1}}}


\newcommand\overmat[2]{%
	\makebox[0pt][l]{$\smash{\color{white}\overbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}^{\text{\color{black}#1}}}$}#2}
\newcommand\bovermat[2]{%
	\makebox[0pt][l]{$\smash{\overbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}^{\text{#1}}}$}#2}
					
\newcommand\bundermat[2]{%
	\makebox[0pt][l]{$\smash{\underbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}_{\text{#1}}}$}#2}
					
					
\newcommand\partialphantom{\vphantom{\frac{\partial e_{P,M}}{\partial w_{1,1}}}}

\usepackage{amsmath}
\usepackage{accents}
\newlength{\dhatheight}
\newcommand{\doublehat}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \smash{\hat{#1}}}


\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}

\newcommand{\systemFGPT}{{FrugalGPT}}


\newcommand{\prompt}{p}
\newcommand{\query}{q}
\newcommand{\answer}{a}
\newcommand{\cost}{c}

%\usepackage{soul}

\usepackage{tcolorbox}

\usepackage[linesnumbered,ruled,vlined]{algorithm2e}


==> theory_backup.tex <==

\section{\GPTNet}\label{LMNet:sec:theory}

\subsection{Analysis of  Modeling of  \LMNet}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figure/example.pdf}
    \caption{An example of \LMNet{}. Given a query $q$, three generators $G_1, G_2, G_3$ generate their answers independently. Next, judges $J_1, J_2$ take these answers as input and then select the most likely answer. Finally, an aggregation function is invoked to obtain the final response $\hat{a}$.}
    \label{fig:LMNet:Example}
\end{figure}

Our goal is to characterize the quality of an \LMNet{}'s answer to a user query. 

\subsection{System Model}
Let us start by considering a specific form of \LMNet{} which consists of three building blocks: a generator, a selector, and a fuser. As shown in  A generator $G_i(\cdot): Q \mapsto A$ takes a query $q\in Q$ as input and generates a candidate answer $a_i\in A$. Given a user query and $m$ candidate answers $a_1,a_2,\cdots, a_m$, an answer selector $S_j(\cdot): Q \times A^{m} \mapsto A $ returns a selected answer $b_j$. A fuser $F(\cdot): A^K \mapsto A$ takes $K$ answers and then aggregates them to produce a final output.

\begin{equation}\label{eq:LMNet:Problem}
    \begin{split}
        a_i & = G_i(q), i=1,2,\cdots, m\\
        b_j & = S_j(q,a_1,a_2,\cdots, a_m), j=1,2,\cdots, K\\
        \hat{a} &= F(b_1,b_2,\cdots,b_K)
    \end{split}
\end{equation}

We consider a $m\times K$ \LMNet{} as described by system equations (\ref{eq:LMNet:Problem}).
In particular, given a query, we first send it to $m$ independent generators to obtain candidate answers. Next, all answers are sent to $K$ separate selectors, each of which gives a selected answer.
Finally, a fuser aggregates all selected answers to a final output. 

To obtain insights on scaling laws for the above \LMNet{}, we need to model the behavior of each component. In particular, we make the following assumptions. 

\begin{assumption}
The answer space is binary, i.e., $A=\{0,1\}$. All generators are independent and return answer  $1$ with probability $p_G$, i.e.,  $a_i\overset{i.i.d}{\sim} \text{Bernoulli}(p_G)$. All selectors are also independent. Furthermore, each selector follows a two-stage answer generation process. First,  it uses the input candidate answers to update its belief on which answer is better. Next, it generates the selected answer via the updated belief. In particular, let $p_S \in [0,1]$ denote a selector's prior on how likely the right answer is $1$. The selector uses a Bayesian rule to update $p_S$, that is, $\frac{1}{2} (p_S+p_G)$, assuming a beta distribution. Finally, the fuser takes a majority vote approach: it computes the average of all inputs, and return 1 if the average is larger than $1/2$ and 0 otherwise.
\end{assumption}


\subsection{Analysis}
Let us start with an asymptotic analysis: Does the \LMNet{}'s performance continuously improve as the number of selectors and generators go to infinity? Surprisingly, the following theorem gives a negative answer.

\begin{theorem}
    Suppose XXX. If $p_G + p_S >1$, then $m,k\rightarrow \infty$ implies that $Pr[a^*=\hat{a}] \rightarrow 1$. On the other hand, if $p_G + p_S <1$, then $m,k\rightarrow \infty$ implies that $Pr[a^*=\hat{a}] \rightarrow 0$.
\end{theorem}

 
In other words, when the sum of the success rate of the selector and the generator is larger than 1, increasing the number of generators and selectors leads to better response quality. If the sum is smaller than 1, then adding more generators and selectors is only a waste of resources. 
This theorem effectively gives a dichotomy on \LMNet{}'s scaling laws.



\paragraph{Examples.} Suppose $p_G=0.3$ and $p_S=0.8$. Then \LMNet{} with an increasingly large number of selectors and generators gives a correct answer with a large probability. In this case, \LMNet{} is better than querying a generator once. Note that, the standard jury approach~\cite{} is worse than querying a generator once in this case. This is because the selector's quality is higher than a naive voting. Thus, even if the majority of candidate answers are incorrect, we can still find the correct ones. 


Suppose $p_G=0.7$ and $p_S=0.4$. This corresponds to another scenario: the generator is of high quality, but the selector is not. Yet, since there are enough high-quality answers, we can still pick up the high-quality answers. 


Suppose $p_G=p_S=0.4$. This is a hard case. Both generators and selectors are not reliable. In such cases, asking a generator alone is actually better than scaling the \LMNet{}.

\paragraph{Limitation and Next Steps.} First, this is only an asymptotic analysis. Finite-sample analysis is crucial in practice. Second, this modeling assumes a specific form of \LMNet{}. How about other ones potentially with more depths and/or other components? Third, this analysis is based on the simplification of the generation space. How does it generalize to other cases, e.g., the generative settings? Fourth, all generators and selectors are considered homogeneous, but this does not hold in practice. I.e., some generators are better than others. How to take this into account? We can explore these directions in the next few days. 




\newpage
\newpage

\subsection{Building block Modeling}
Let us start by modeling each building block in \LMNet{}.  

Generator: Each generator's answer $\hat{a}_i$ matches the desired answer with probability $p$. 

Judge: Each judge is responsible for generating an answer after reading all generators' answers. Here, let us consider a particular judge form: Bayesian judge. In particular, it encodes all generators' answers as prior knowledge and uses it to update its own generation.

Aggregator: Aggregator gets all information from them.




\begin{equation}
    \hat{a}_i = a \text{ w.p. $p$}
\end{equation}

\begin{equation}
    \sum_{i=1}^{m} \hat{a}_i
\end{equation}


A generator $G_i(\cdot): Q \mapsto A$ takes a query $q\in Q$ as input and generates an answer $a_i\in A$. 


Given a user query and $m$ possible answers from , an answer selector $S_j(\cdot): Q \times A^{m} \mapsto A $ maps 


\subsection{Another modeling}

Capacity v.s. Randomness.



\subsection{Performance Analysis on A \deluxechat{} Instance}
When and why can \deluxechat{} generate answers better than individual generators? We give a formal analysis on a simple instance of \deluxechat{} called $(p_{g,1},p_{g,2},p_s)$ independent \deluxechat{}. 

\begin{definition}
    A \deluxechat{} instance $F$ is called $(p_{g,1},p_{g,2},p_s)$ independent if  
    \begin{itemize}
        \item it has 2 answer generators, $G_1$ and $G_2$,
        \item the two generators and the selector are independent,
        \item generators give  a high-quality answer with probability $p_{g,1},p_{g,2}$ respectively,
        \item selector recognizes the better answer with probability $p_s$.
    \end{itemize}
\end{definition}

Intuitively, $(p_{g,1},p_{g,2},p_s)$ independence focuses on \deluxechat{} with two answer generators. Roughly speaking, the independence assumption ensures that generators are \textit{complementary}, i.e., different LMs perform the best on different user queries. For this \deluxechat{} instance, we can precisely quantify how good the selector must be to ensure $(p_{g,1},p_{g,2},p_s)$ independent \deluxechat{} is better than any individual generator it uses. 


\begin{theorem}\label{thm:deluxechat:selectorquality}
    Suppose $F$ is $(p_{g,1},p_{g,2},p_s)$ independent. Then we have 
    \begin{equation*}
        \Pr[s(\pmb x, F(\pmb x))=1] > \max_{i\in\{1,2\}} \Pr[s(\pmb x, G_i(\pmb x))=1]
    \end{equation*}
    if and only if 
    \begin{equation*}
        p_s >\frac{1}{1+\frac{1-\max_{i}p_{g,i}}{\max_i \frac{p_{g,i}}{p_{g,3-i}}-\max_{i}p_{g,i}}}.
    \end{equation*}
\end{theorem}

There are several implications of Theorem \ref{thm:deluxechat:selectorquality}. First, the quality of the selector plays an important role in \deluxechat{}. In fact,  \deluxechat{}'s performance is better than that of individual generators only when the selector's quality is higher than the threshold given in Theorem \ref{thm:deluxechat:selectorquality}. As a concrete example, suppose two generators are of the same quality ($p_{g,1}=p_{g,2}$). Then the threshold becomes $\frac{1}{2}$, indicating that the selector needs to be better than random guessing. 
Second, the larger gap between the individual generators' quality, the better the selector needs to be. This is because a large quality gap implies a large value of $\max_i{p_{g, i}/p_{g,3-i}}$, and thus a small value of the denominator of the threshold and a large value of the threshold.
These observations suggest that improving (i) the selector quality or (ii) the quality of the relatively weak generator should lead to performance improvement of \deluxechat{} in practice. 


\subsection{Initial Attempts on Scaling Laws}
Now we offer an initial model to study the scaling laws. To do so, we need to first model the generator and the selector in a more fine-grained way.

Generator: $g(\cdot,\cdot)$, where the first parameter encodes the input query, and the second parameter denotes the generation prompt.



Selector: $s(\cdot,\cdot,\cdot)$ The first two are the input answers to compare, and the last is the noise of the selector.


\paragraph{Scaling option 1: adding more selector.}


\newpage
\section{\LMNet{}}
In this section, we introduce and analyze the framework of \LMNet{}. In particular, we would start by defining \LMNet{} formally, then give some common examples of \LMNet{}, and finally analyze and compare the performance of some \LMNet{} instances. 

\subsection{What is \LMNet{}?}
Mathmetically, \LMNet{} is a directed acyclic graph (DAG), where each node is one \LM{}, and each edge indicates how information flows between different \LM{}s. Specifically, an edge pointing to a node represents one input, and an edge pointing out from a node is an output. An node is an \LM{} that transforms (multiple) inputs as (multiple) outputs. Note that a node is determined not only by its inputs, outputs, and \LM{} instances (GPT-4, Claude-2, Llamma, etc), but also its model parameters such as prompts and temperatures.  

\LMNet{} is a generic framework that subsumes many existing concepts and techniques to use. For concreteness, we consider only a few types of nodes in this paper. 

\paragraph{generator.} A generator node is denoted by $g(\cdot,\cdot)$. Here, the first parameter is the input to process, and the second parameter denotes the model parameters,  such as system prompts and temperatures. Intuitively, a generator node is responsible for generating a possible answer to a user query. 


\paragraph{selector.} A selector node is denoted by $s(\cdot,\cdot,\cdot, \cdot)$, where the first parameter represents the user query, the second and third parameters denote two candidate answers, and the last parameter again is the model parameters. The output of a selector is one of the two candidate answers, potentially with some explanations.   %An selector is responsible to select which generation to trust. 

\subsection{\LMNet{} Instances}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figure/InferenceNetwork_flow.pdf}
    \caption{Illustration of the \LMNet{} instances.}
    \label{fig:GPTNet}
\end{figure}
How does a \LMNet{} consisting of only generators and selectors work? While seemingly simple, this has already allowed many interesting \LMNet{} instances.

\paragraph{Warm-up: A two-layer \LMNet{}.} Let us first consider the following simple \LMNet{}.

\begin{align*}
    &r_1 = g(x,\epsilon_1)\\
    &r_2 = g(x,\epsilon_2)\\
    &F_2(x) = s(x, r_1, r_2,\delta)\\
\end{align*}
Here, $x$ is the user query, $\epsilon_1$ and $\epsilon_2$ are the model parameters for the generators, and $\delta$ is the model parameter for the selector.

\paragraph{Selector-scaling \LMNet{}.} Now let us consider a more complicated instance that scaling up the number of selectors. Specifically, it first uses two generators to create two possible answers. Next, it uses two separate selectors to refine the answers, and keep this process for $n$ times. Finally, the output is simply the output from the last selector. This can be formally described by the following equations.  
\begin{align*}
    r_{1,i} &= g(x,\epsilon_{1,i}),i=1,2\\
    r_{k,i} & = s(x, r_{k-1,1}, r_{k-1,2}, \delta_{k,i}), i=1,2, k=2,\cdots, n\\
    F_{s,n}(x) & = r_{n,1}
\end{align*}
Again, $\epsilon_{k,i}$ represent model parameters for the generators, and $\delta_{k,i}$ denote model parameters for the selectors.

\paragraph{Generator-scaling \LMNet{}.} Next let us consider the dual approach to scale up the two-layer \LMNet{}: generator-scaling. In particular, it initializes its answer by querying one generator. 
Next, it updates the answer by (i) generating a new answer, and (ii) comparing it with the current answer by the selector.
This is repeated $n$ times, and then it returns the final answer.  The following system of equations precisely quantifies this \LMNet{}. 

\begin{align*}
    r_1 &= g(x,\epsilon_1)\\
    r'_{k} & = g(x,\epsilon_k), k=2,\cdots, n\\
    r_k & = s(x, r_{k-1}, r_{k}', \delta_k), k=2,\cdots, n\\
    F_{g,n}(x) & = r_n
\end{align*}
Similarly, $\epsilon_{k}$ represent model parameters for the generators, and $\delta_{k}$ denotes model parameters for the selectors.

\subsection{Asymptotic Performance Analysis of \LMNet{}}
Which \LMNet{} should one use? When and why does one \LMNet{} instance outperform another one? Answers to these questions heavily depend on the model parameters for the selectors and the generators. Suppose, for example, the model parameters are always perfect (e.g., they directly encode the correct answer), then the simple two-layer \LMNet{} is sufficient. Therefore, we need to characterize the quality of the model parameters. 

\begin{theorem}
Suppose $\epsilon_1,\epsilon_2$ are iid. And in addition, $\Pr[ q(x,g(x,\epsilon_{1}))=1 ] = p_{g,1}$, $\Pr[ q(x,g(x,\epsilon_{1}))=1 ] = p_{g,2}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=1,q(a_2)=0 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=0,q(a_2)=1 ] = p_{s}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=1,q(a_2)=1 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=0| q(a_1)=0,q(a_2)=0 ] = 1$. W.L.O.G, assume $p_{g,1}\geq p_{g,2}$. Then we have 
    \begin{equation*}
        \Pr[q(\pmb x, F_2(\pmb x))=1] >  \Pr[q(\pmb x, g(\pmb x,\epsilon_1))=1]
    \end{equation*}
    if and only if 
    \begin{equation*}
        p_s >\frac{1}{1+\frac{1-p_{g,1}}{\alpha-p_{g,2}}}.
    \end{equation*}
\end{theorem}
Basically, this says that the two-layer \LMNet{} needs high-quality selector in order to be better than using the better individual generator.

\begin{theorem}
Suppose all model parameters $\epsilon_{k,i}, \delta_{k,i}$ are i.i.d. And in addition, $\Pr[ q(x,g(x,\epsilon_{k,i}))=1 ] = p_{g}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=1,q(a_2)=0 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=0,q(a_2)=1 ] = p_{s}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=1,q(a_2)=1 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=0| q(a_1)=0,q(a_2)=0 ] = 1$. Then we have 
\begin{align*}
   &\Pr[q(x, \lim_{n\mapsto \infty} F_{s,n}(x))=1 ] \\=&p_g^2+ 2p_g (1-p_g) \frac{p_s^2}{p_s^2+(1-p_s)^2}
\end{align*}
\end{theorem}


\begin{theorem}
Suppose all model parameters $\epsilon_{k}, \delta_{k}$ are i.i.d. And in addition, $\Pr[ q(x,g(x,\epsilon_{k}))=1 ] = p_{g}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k}))=1| q(a_1)=1,q(a_2)=0 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=0,q(a_2)=1 ] = p_{s}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=1,q(a_2)=1 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=0| q(a_1)=0,q(a_2)=0 ] = 1$. Then we have 
\begin{align*}
   &\Pr[q(x, \lim_{n\mapsto \infty} F_{g,n}(x))=1 ] \\=&\frac{p_sp_g}{p_s p_g + (1-p_g)(1-p_s)}
\end{align*}
\end{theorem}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figure/NetCompare.png}
    \caption{Performance differences between the selector network and the generator network.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figure/fitscalelaw.png}
    \caption{Fitting scale laws on the commonsenseqa.}
    \label{fig:enter-label}
\end{figure}

\begin{theorem}[Characterization of network] If $p_g\in\{0,1\}$ or $p_s=\frac{1}{2}$ or $p_s=p_g$, then $\Pr[q(x, \lim_{n\mapsto \infty} F_{s,n}(x))=1 ] = \Pr[q(x, \lim_{n\mapsto \infty} F_{g,n}(x))=1 ]$. If $0<p_g<1, p_s\not=\frac{1}{2}$ and $p_s\not=p_g$, then we have $\Pr[q(x, \lim_{n\mapsto \infty} F_{s,n}(x))=1 ] > \Pr[q(x, \lim_{n\mapsto \infty} F_{g,n}(x))=1 ]$ if and only if $p_g>p_s$.

\end{theorem}
\begin{proof}
    Note that 
    \begin{align*}
   &\Pr[q(x, \lim_{n\mapsto \infty} F_{s,n}(x))=1 ] > \Pr[q(x, \lim_{n\mapsto \infty} F_{g,n}(x))=1 ]
\end{align*}
is equivalent to 
\begin{align*}
   &p_g^2+ 2p_g (1-p_g) \frac{p_s^2}{p_s^2+(1-p_s)^2} > \frac{p_sp_g}{p_s p_g + (1-p_g)(1-p_s)}
\end{align*}
The denominators on both sides are non-negative. Thus, we can multiply both sides by $p_s p_g + (1-p_g)(1-p_s)$ and $p_s^2+(1-p_s)^2$ and obtain 
\begin{align*}
    [p_s p_g + (1-p_g)(1-p_s)][2p_g (1-p_g)p_s^2 +p_g^2(p_s^2+(1-p_s)^2)] > p_s p_g [p_s^2+(1-p_s)^2]
\end{align*}
Let $H(p_s,p_g) \triangleq [p_s p_g + (1-p_g)(1-p_s)][2p_g (1-p_g)p_s^2 +p_g^2(p_s^2+(1-p_s)^2)] - p_s p_g [p_s^2+(1-p_s)^2]$. Thus, 
\begin{align*}
   &\Pr[q(x, \lim_{n\mapsto \infty} F_{s,n}(x))=1 ] > \Pr[q(x, \lim_{n\mapsto \infty} F_{g,n}(x))=1 ]
\end{align*}
if and only if $H(p_s,p_g)>0$. 
Now let us consider $H(p_s,p_g)$. Suppose $p_g>0$. Then we can divide $H(p_s,p_g)$ by $p_g$ to obtain
\begin{align*}
\frac{H(p_s,p_g)}{p_g} = [p_s p_g + (1-p_g)(1-p_s)][2 (1-p_g)p_s^2 +p_g(p_s^2+(1-p_s)^2)] - p_s [p_s^2+(1-p_s)^2]    
\end{align*}
Now, let us view $p_s$ as a constant and $p_g$ as a variable, and then rearrange the terms to obtain 
\begin{align*}
\frac{H(p_s,p_g)}{p_g} & = [p_s p_g + (1-p_g)(1-p_s)][2 (1-p_g)p_s^2 +p_g(p_s^2+(1-p_s)^2)] - p_s [p_s^2+(1-p_s)^2]    \\
&= [(2p_s-1) p_g +(1-p_s)][ p_g(p_s^2+(1-p_s)^2-2p_s^2) + 2 p_s^2] - p_s [p_s^2+(1-p_s)^2] \\
&= [(2p_s-1) p_g +(1-p_s)][ (1-2p_s) p_g + 2 p_s^2] - p_s [p_s^2+(1-p_s)^2]
\end{align*}
Now expanding all terms in the first product gives
\begin{align*}
\frac{H(p_s,p_g)}{p_g} 
&= [(2p_s-1) p_g +(1-p_s)][ (1-2p_s) p_g + 2 p_s^2] - p_s [p_s^2+(1-p_s)^2] \\
&= -(1-2p_s)^2 p_g^2 +  [(2p_s-1)2p_s^2+(1-2p_s)(1-p_s)] p_g + (1-p_s) 2p_s^2 - p_s [p_s^2+(1-p_s)^2]
\end{align*}
Now we can rewrite this equality as 
\begin{align*}
\frac{H(p_s,p_g)}{p_g} 
&= -(1-2p_s)^2 p_g^2 +  [(2p_s-1)2p_s^2+(1-2p_s)(1-p_s)] p_g + (1-p_s) 2p_s^2 - p_s [p_s^2+(1-p_s)^2]\\
&=  -(1-2p_s)^2 p_g^2 +  (1-2p_s)(1-p_s-2p_s^2) p_g - p_s [p_s^2+(1-p_s)^2-2p_s(1-p_s)]\\
&=  -(1-2p_s)^2 p_g^2 +  (1-2p_s)(1-p_s-2p_s^2) p_g - p_s (1-2p_s)^2\\
&= -(1-2p_s) [(1-2p_s)p_g^2 - (1-p_s-2p_s^2) p_g +p_s (1-2p_s)]\\
&= -(1-2p_s) [(1-2p_s)p_g^2 - (1-2p_s)(1+p_s) p_g +p_s (1-2p_s)]\\
&= -(1-2p_s)^2  
[p_g^2-(1+p_s)p_g+p_s]\\
&= -(1-2p_s)^2  (p_g-p_s)(p_g-1)
\end{align*}
Here, the second equality is by expanding all terms, the third equality is by algebraic rewriting the third term from the last equation, the fourth equation extracts the common factor $1-2p_s$, the fifth equation uses the fact that $1-a-2a^2=(1+a)(1-2a)$, the sixth equation extract the common factor $1-2p_s$ again, and the final equation uses the fact that $a^2-(1+b)a+b=(a-b)(a-1)$.
Therefore, we have shown that 
\begin{align*}
    H(p_s,p_g) = - p_g (1-2p_s)^2 (p_g-p_s) (p_g-1)
\end{align*}
$H(p_s,p_g)>0$ if and only if $0<p_g<1,p_s\not=\frac{1}{2}, p_g >p_s$. 
\end{proof}

\subsection{Finite sample analysis}
How does the performance scale as a function of the number of generators and selectors? At least we can have a simulation-based analysis.

Selector Net: 

\begin{align*}
    q(F_{s,n}(x)) = [1,\frac{1}{2}, 0] S^n\begin{pmatrix}
        p_g^2\\
        2p_g(1-p_g)\\
        (1-p_g)^2\\
    \end{pmatrix} 
\end{align*}

Generator Net:
\begin{align*}
    q(F_{g,n}(x)) = [1,0]\left[G^n \begin{pmatrix}
        p_g\\
        1-p_g
    \end{pmatrix}\right]
\end{align*}
where
\begin{align*}
G = \begin{pmatrix}
p_g + (1 - p_g) p_s & p_g p_s \\
(1 - p_g) (1 - p_s) & 1 - p_s p_g
\end{pmatrix}
\end{align*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/finite_analysis.pdf}
    \caption{Finite sample analysis on the generator and selector net.}
    \label{fig:enter-label}
\end{figure}
\subsection{modeling selectors with multiple inputs}
The selector quality depends on two factors, (i) $n$ the number of inputs, and (ii) $r$ the fraction of correct answers.

The probability of getting a correct answer is 
\begin{align}
    p_{n,r} = \alpha(n) +r^{\beta(n)} (1-\alpha(n))
\end{align}
where 
\begin{align}
    \alpha(n) = \exp(-(n-z)^2)
\end{align}
and 
\begin{align}
    \beta(n) = \exp(-\gamma n)
\end{align}


Another simplified model is 
\begin{align*}
    P_{n,r} = [(1-c) r + c]^{a \log n +b }
\end{align*}
\subsection{Some research questions to answer}
\begin{itemize}
    \item How do these analytical models match the empirical results?
    \item How to connect the hierarchical scaling with multiple-input selector's scaling?
    \item How do we justify the multiple-input selector' model?
    \item How to extend the asymptotic analysis to finite sample analysis? 
\end{itemize}


\section{An analytical model to explain the U shape}
By contrast to the traditional wisdom on scaling laws of training data and model parameters, the experiments shown in Figure \ref{} suggest that \LMNet{}'s performance is not necessarily monotone w.r.t. the number of network components. Why is this the case? In this section, we offer an analytical model to explain this phenomenon. The key insight is that, in a nutshell, the data matters.


\subsection{System models}
Let us consider a simple network: given a query $x$, we generate $K$ candidate answers $z_1, z_2, \cdots, z_K$, and then take the majority vote as the final response. Suppose all $z_i$ are generated independently from some population, and let $p_x$ be the probability of the answer being correct. Let $f(x;k)$ denote the probability of the final answer being correct and let us denote the log-likelihood $F(k;D) \triangleq \mathbb{E}_{x\sim D} [\log f(x;k)]$ as the loss function. 
As a first step, let us consider binary prediction tasks, and when it is clear from the context, let us 

Now our question is, How does $F(k;D)$ scale as a function of $k$?

\subsection{Scaling laws for a fixed $x$}
Let us start by considering how $f(x;k)$ scales. W.L.O.G, suppose the correct answer is $1$, and then the majority vote network is correct when 
\begin{align*}
    \frac{1}{K}\sum_{K}^{i=1}z_i > \frac{1}{2}
\end{align*}
Noting that $z_i$ is correct with probability $p_x$, we can rewrite the above as 

\begin{align*}
    \frac{1}{K}\sum_{K}^{i=1}z_i - p_x > \frac{1}{2} - p_x
\end{align*}

Suppose $p_x>\frac{1}{2}$. The above event implies $|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| < p_x - \frac{1}{2}$. Applying 
Hoeffding's inequality gives that 
\begin{align*}
\Pr[|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| < p_x - \frac{1}{2}] \geq 1-2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}
Thus, we have 
\begin{align*}
    f(x;k) = \Pr[\frac{1}{K}\sum_{K}^{i=1}z_i>\frac{1}{2}] \geq  1 - 2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}

Suppose $p_x<\frac{1}{2}$. Then the above event implies $|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| > \frac{1}{2}-p_x$. Now applying Hoeffding's inequality gives us that 
\begin{align*}
\Pr[|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| > 1/2- p_x ] \leq 2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}
That is, 
\begin{align*}
    f(x;k) = \Pr[\frac{1}{K}\sum_{K}^{i=1}z_i>\frac{1}{2}] \leq  2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}
To sum up, we have the following result
\begin{align*}
    f(x;k) \begin{cases}
        \geq   1 - 2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x >\frac{1}{2}\\
        \leq 2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x < \frac{1}{2}
    \end{cases}
\end{align*}

For large $K$, Hoeffding's inequality is ``tight'', and thus we can approximate the above inequalities by equality and obtain 

\begin{align*}
    f(x;k) \approx g(x;k) \triangleq \begin{cases}
        1 - 2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x >\frac{1}{2}\\
         2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x < \frac{1}{2}
    \end{cases}
\end{align*}
This gives a scaling law that depends on the given problem: if the problem is easy, i.e., most samples are correct ($p_x > \frac{1}{2}$), then generating more candidate answers improves the performance. if the problem is hard, i.e., most samples are incorrect ($p_x < \frac{1}{2}$), adding more candidate answers lowers the performance!

\subsection{Scaling laws for $F(k;D)$}
The previous section suggests that for fixed query $x$,  enlarging the network monotonically improves or worsens the performance, depending on the difficulty of the query $x$. In practice, the problem difficulty is diverse. Therefore, there is a balance between easy and hard problems: easy problems need more candidate answers, but hard problems want fewer. This intuitively explains why empirically the scaling performance is non-monotone. 

Now let us make the above intuition formal by quantifying the loss function. This is, of course, intractable for general data distribution $D$. For simplicity, let us consider a simple instance $D(p_1, p_2, \alpha)$. Here, the data distribution is a mixture of two distributions. All problems in the first is easy with correct probability $p_x=p_1>\frac{1}{2}$. And the second distribution contains hard problems, where each candidate answer is correct with probability $p_x=p_2<\frac{1}{2}$. $\alpha$ is the fraction of samples from the first distribution. Now let us expand $F(K;D)$ as
\begin{align*}
    F(K;D) = &\mathbb{E}_{x\sim D} \log f(x;K) \approx G(K;D) = \mathbb{E}_{x\sim D} \log g(x;K) \\
    =& \alpha \log  [1-2 \exp(-\frac{2(p_1-1/2)^2}{K})]  + (1-\alpha)\log[2 \exp(-\frac{2(p_2-1/2)^2}{K}]) \\
    = & \alpha \log  [1-2 \exp(-\frac{2(p_1-1/2)^2}{K})]  - \frac{2(1-\alpha)(p_2-1/2)^2}{K} + (1-\alpha) \log 2\\
\end{align*}

This is the scaling law of the loss as a function of the number of candidate answers for distribution $D(p_1,p_2,\alpha)$. 
While simple, this also sheds light on scaling laws for general distributions $D$. In fact, one can approximate any distribution $D$ by discretizing the value of an candidate answer being correct, and in general, we can make this an integral. 

\subsection{Optimal candidate answer size}
What is the optimal candidate answer size? Let us keep studying the above distribution instance. By COV, let $M\triangleq\frac{1}{K}$, we can rewrite it as  

\begin{align*}
    G(1/M;D) 
    = & \alpha \log  [1-2 \exp(-2(p_1-1/2)^2M)]  - 2(1-\alpha)(p_2-1/2)^2M + (1-\alpha) \log 2\\
\end{align*}
The first term is concave, the second term is linear in $M$, and hence the above is concave in $G$. Therefore, any stationary points are optimal. Let us take the derivative 

\begin{align*}
    \partial \frac{G(1/M;D)}{\partial M} 
    = & \alpha \frac{-4(p_1-1/2)^2 \exp(-2(p_1-1/2)^2M)}{1-2 \exp(-2(p_1-1/2)^2M)}   - 2(1-\alpha)(p_2-1/2)^2\\
\end{align*}
Let $W = \exp(-2(p_1-1/2)^2M)$.
Then above is 
\begin{align*}
    \partial \frac{G(1/M;D)}{\partial M} 
    = & \alpha \frac{4(p_1-1/2)^2 W)}{1-2 W}   - 2(1-\alpha)(p_2-1/2)^2\\
\end{align*}
$ \frac{\partial G(1/M;D)}{\partial M} =0$ implies 

\begin{align*}
    W = \frac{c_2}{\alpha c_1+2 c_2}
\end{align*}
where $c_1 = 4(p_1-1/2)^2$ and $c_2 = 2(1-\alpha) (p_2-1/2)^2$.

Now map $W$ back to $K$ we have
\begin{align*}
    K^* = \frac{-2(p_1-1)^2}{\log \frac{c_2}{\alpha c_1 +2 c_2}}
\end{align*}

Note that, interestingly, the solution is unique and positive. It is not hard to prove that, $G(K;D)$ increases until $K=K^*$ and then it decreases. This matches the empirical observations.  

\subsection{Fitting the scaling laws }
There are many ways to fit the scaling laws for a real-world problem. here we list two of them.

\paragraph{Problem Difficulty Estimation.} The key observation of the non-monotone scaling comes from problem difficulty heterogeneity. Thus, a natural idea is to estimate the problem's difficulty first and then plug in the values $p_1, p_2$ in the scaling laws. More generally, as we mentioned before, one can use other parametric versions of the data hardness to fit this. 

\paragraph{Direct estimation Formula fitting.} Note that our goal is to predict $F(K;D)$ while all analysis is assume $F(K;D)\approx G(K;D)$. That is to say, even if the difficulty estimation is perfect, the plugging-in approach may not be accurate as well. Thus, an alternative approach is to directly estimate the parameters in the scaling law.
Recall that the scaling law is
\begin{align*}
    G(K;D)
    = & \alpha \log  [1-2 \exp(-\frac{2(p_1-1/2)^2}{K})]  - \frac{2(1-\alpha)(p_2-1/2)^2}{K} + (1-\alpha) \log 2\\
\end{align*}
And W.L.O.G, we can simply rewrite it as 
\begin{align*}
    G(K;D)
    = & c_1  \log  [1-c_2 \exp(-\frac{c_3}{K})]  - \frac{c_3}{K} + c_4\\
\end{align*}
Now, we can use training data to fit the constant $c_1,c_2,c_3,c_4$, and then directly predict the scaling law. One benefit here is that, this can hopefully mitigate the approximation error $F(K;D)-G(K;D)$ 

\subsection{What experiments to run?}
We need to verify this asusmp

TODO: cleaning the remaining. 
\newpage

\subsection{Building Blocks}

Generator: $g(\cdot,\cdot)$, where the first parameter encodes the input query, and the second parameter denotes the generation prompt.



Selector: $s(\cdot,\cdot,\cdot,\cdot)$. The first is the input query,  The second two are the two candidate answers to compare, and the last is the selector prompt.


\subsection{The Two layer \LMNet{}: A warm-up}
Let us consider a warm-up example. 



\subsection{Scaling up the selectors}
\begin{align*}
    r_{1,i} &= g(x,\epsilon_{1,i}),i=1,2\\
    r_{k,i} & = s(x, r_{k-1,1}, r_{k-1,2}, \delta_{k,i}), i=1,2\\
    \hat{r} & = r_{n,1}
\end{align*}


\subsection{Scaling up the generators}


\begin{align*}
    r_1 &= g(x,\epsilon_1)\\
    r'_{k} & = g(x,\epsilon_k)\\
    r_k & = s(x, r_{k-1}, r_{k}', \delta_k)\\
    \hat{r} & = r_n
\end{align*}

How do we measure the quality? 

\begin{align*}
    \Pr[q(\hat{r},x)=1]
\end{align*}


Assumptions:
\begin{itemize}
    \item $\epsilon, \delta$ are i.i.d.
    \item $\Pr[]$
\end{itemize}


\begin{theorem}
    $\Pr[q(r_s)=1] = p_g^2+2p_g(1-p_g) \frac{p_s^2}{p_s^2+(1-p_s)^2}$
\end{theorem}
\subsection{}



\section{TODOs}

\subsection{Scaling laws for a fixed $x$}
Let us start by considering how $f(x;k)$ scales. W.L.O.G, suppose the correct answer is $1$, and then the majority vote network is correct when the most candidate answers are correct. That means the probability of being correct is
\begin{align*}
    f(x;K) = \Pr\left[\frac{1}{K}\sum^{K}_{i=1}z_i > \frac{1}{2}\right]
\end{align*}
All $z_i$ are i.i.d, and each one is one with probability $p_x$. Therefore, their sum is a binomial distribution, and thus the above can be written as, for simplicity, assuming $K$ is odd, we have
\begin{align*}
    f(x;K) = 1- \Pr\left[\sum^{K}_{i=1}z_i \leq \frac{K}{2}\right] = 1 - I_{1-p_x}(K-(K-1)/2, 1+(K-1)/2) =  I_{p_x}((K+1)/2, (K+1)/2)
\end{align*}
where $I(\cdot)\triangleq $ is the regularized incomplete beta function.

\subsection{Scaling laws for a dataset $D$} 
The loss is simply 
\begin{align*}
    F(D;K) = \mathbb{E}_{x\sim D} [\ell (f(x;K))] = \int_{0}^{1} \ell (f(x;K)) q(p_x) d p_x = \int_{0}^{1} I_{p_x} ((K+1)/2, (K+1)/2) q(p_x) d p_x 
\end{align*}


Let us start by considering how $f(x;k)$ scales. W.L.O.G, suppose the correct answer is $1$, and then the majority vote network is correct when 
\begin{align*}
    \frac{1}{K}\sum_{K}^{i=1}z_i > \frac{1}{2}
\end{align*}
Noting that $z_i$ is correct with probability $p_x$, we can rewrite the above as 

\begin{align*}
    \frac{1}{K}\sum_{K}^{i=1}z_i - p_x > \frac{1}{2} - p_x
\end{align*}

Suppose $p_x>\frac{1}{2}$. The above event implies $|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| < p_x - \frac{1}{2}$. Applying 
Hoeffding's inequality gives that 
\begin{align*}
\Pr[|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| < p_x - \frac{1}{2}] \geq 1-2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}
Thus, we have 
\begin{align*}
    f(x;k) = \Pr[\frac{1}{K}\sum_{K}^{i=1}z_i>\frac{1}{2}] \geq  1 - 2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}

Suppose $p_x<\frac{1}{2}$. Then the above event implies $|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| > \frac{1}{2}-p_x$. Now applying Hoeffding's inequality gives us that 
\begin{align*}
\Pr[|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| > 1/2- p_x ] \leq 2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}
That is, 
\begin{align*}
    f(x;k) = \Pr[\frac{1}{K}\sum_{K}^{i=1}z_i>\frac{1}{2}] \leq  2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}
To sum up, we have the following result
\begin{align*}
    f(x;k) \begin{cases}
        \geq   1 - 2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x >\frac{1}{2}\\
        \leq 2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x < \frac{1}{2}
    \end{cases}
\end{align*}

For large $K$, Hoeffding's inequality is ``tight'', and thus we can approximate the above inequalities by equality and obtain 

\begin{align*}
    f(x;k) \approx g(x;k) \triangleq \begin{cases}
        1 - 2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x >\frac{1}{2}\\
         2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x < \frac{1}{2}
    \end{cases}
\end{align*}
This gives a scaling law that depends on the given problem: if the problem is easy, i.e., most samples are correct ($p_x > \frac{1}{2}$), then generating more candidate answers improves the performance. if the problem is hard, i.e., most samples are incorrect ($p_x < \frac{1}{2}$), adding more candidate answers lowers the performance!

\subsection{Scaling laws for $F(k;D)$}
The previous section suggests that for fixed query $x$,  enlarging the network monotonically improves or worsens the performance, depending on the difficulty of the query $x$. In practice, the problem difficulty is diverse. Therefore, there is a balance between easy and hard problems: easy problems need more candidate answers, but hard problems want fewer. This intuitively explains why empirically the scaling performance is non-monotone. 

Now let us make the above intuition formal by quantifying the loss function. This is, of course, intractable for general data distribution $D$For simplicity, let us consider a simple instance $D(p_1, p_2, \alpha)$. Here, the data distribution is a mixture of two distributions. All problems in the first is easy with correct probability $p_x=p_1>\frac{1}{2}$. And the second distribution contains hard problems, where each candidate answer is correct with probability $p_x=p_2<\frac{1}{2}$. $\alpha$ is the fraction of samples from the first distribution. Now let us expand $F(K;D)$ as
\begin{align*}
    F(K;D) = &\mathbb{E}_{x\sim D} \log f(x;K) \approx G(K;D) = \mathbb{E}_{x\sim D} \log g(x;K) \\
    =& \alpha \log  [1-2 \exp(-\frac{2(p_1-1/2)^2}{K})]  + (1-\alpha)\log[2 \exp(-\frac{2(p_2-1/2)^2}{K}]) \\
    = & \alpha \log  [1-2 \exp(-\frac{2(p_1-1/2)^2}{K})]  - \frac{2(1-\alpha)(p_2-1/2)^2}{K} + (1-\alpha) \log 2\\
\end{align*}

This is the scaling law of the loss as a function of the number of candidate answers for distribution $D(p_1,p_2,\alpha)$. 
While simple, this also sheds light on scaling laws for general distributions $D$. In fact, one can approximate any distribution $D$ by discretizing the value of an candidate answer being correct, and in general, we can make this an integral. 

\subsection{Optimal candidate answer size}
What is the optimal candidate answer size? Let us keep studying the above distribution instance. By COV, let $M\triangleq\frac{1}{K}$, we can rewrite it as  

\begin{align*}
    G(1/M;D) 
    = & \alpha \log  [1-2 \exp(-2(p_1-1/2)^2M)]  - 2(1-\alpha)(p_2-1/2)^2M + (1-\alpha) \log 2\\
\end{align*}
The first term is concave, the second term is linear in $M$, and hence the above is concave in $G$. Therefore, any stationary points are optimal. Let us take the derivative 

\begin{align*}
    \partial \frac{G(1/M;D)}{\partial M} 
    = & \alpha \frac{-4(p_1-1/2)^2 \exp(-2(p_1-1/2)^2M)}{1-2 \exp(-2(p_1-1/2)^2M)}   - 2(1-\alpha)(p_2-1/2)^2\\
\end{align*}
Let $W = \exp(-2(p_1-1/2)^2M)$.
Then above is 
\begin{align*}
    \partial \frac{G(1/M;D)}{\partial M} 
    = & \alpha \frac{4(p_1-1/2)^2 W)}{1-2 W}   - 2(1-\alpha)(p_2-1/2)^2\\
\end{align*}
$ \frac{\partial G(1/M;D)}{\partial M} =0$ implies 

\begin{align*}
    W = \frac{c_2}{\alpha c_1+2 c_2}
\end{align*}
where $c_1 = 4(p_1-1/2)^2$ and $c_2 = 2(1-\alpha) (p_2-1/2)^2$.

Now map $W$ back to $K$ we have
\begin{align*}
    K^* = \frac{-2(p_1-1)^2}{\log \frac{c_2}{\alpha c_1 +2 c_2}}
\end{align*}

Note that, interestingly, the solution is unique and positive. It is not hard to prove that, $G(K;D)$ increases until $K=K^*$ and then it decreases. This matches the empirical observations.  

\subsection{Fitting the scaling laws }
There are many ways to fit the scaling laws for a real-world problem. here we list two of them.

\paragraph{Problem Difficulty Estimation.} The key observation of the non-monotone scaling comes from problem difficulty heterogeneity. Thus, a natural idea is to estimate the problem's difficulty first and then plug in the values $p_1, p_2$ in the scaling laws. More generally, as we mentioned before, one can use other parametric versions of the data hardness to fit this. 

\paragraph{Direct estimation Formula fitting.} Note that our goal is to predict $F(K;D)$ while all analysis is assume $F(K;D)\approx G(K;D)$. That is to say, even if the difficulty estimation is perfect, the plugging-in approach may not be accurate as well. Thus, an alternative approach is to directly estimate the parameters in the scaling law.
Recall that the scaling law is
\begin{align*}
    G(K;D)
    = & \alpha \log  [1-2 \exp(-\frac{2(p_1-1/2)^2}{K})]  - \frac{2(1-\alpha)(p_2-1/2)^2}{K} + (1-\alpha) \log 2\\
\end{align*}
And W.L.O.G, we can simply rewrite it as 
\begin{align*}
    G(K;D)
    = & c_1  \log  [1-c_2 \exp(-\frac{c_3}{K})]  - \frac{c_3}{K} + c_4\\
\end{align*}
Now, we can use training data to fit the constant $c_1,c_2,c_3,c_4$, and then directly predict the scaling law. One benefit here is that, this can hopefully mitigate the approximation error $F(K;D)-G(K;D)$ 



\subsection{Analysis of  Modeling of  \LMNet}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figure/example.pdf}
    \caption{An example of \LMNet{}. Given a query $q$, three generators $G_1, G_2, G_3$ generate their answers independently. Next, judges $J_1, J_2$ take these answers as input and then select the most likely answer. Finally, an aggregation function is invoked to obtain the final response $\hat{a}$.}
    \label{fig:LMNet:Example}
\end{figure}

Our goal is to characterize the quality of an \LMNet{}'s answer to a user query. 

\subsection{System Model}
Let us start by considering a specific form of \LMNet{} which consists of three building blocks: a generator, a selector, and a fuser. As shown in  A generator $G_i(\cdot): Q \mapsto A$ takes a query $q\in Q$ as input and generates a candidate answer $a_i\in A$. Given a user query and $m$ candidate answers $a_1,a_2,\cdots, a_m$, an answer selector $S_j(\cdot): Q \times A^{m} \mapsto A $ returns a selected answer $b_j$. A fuser $F(\cdot): A^K \mapsto A$ takes $K$ answers and then aggregates them to produce a final output.

\begin{equation}\label{eq:LMNet:Problem}
    \begin{split}
        a_i & = G_i(q), i=1,2,\cdots, m\\
        b_j & = S_j(q,a_1,a_2,\cdots, a_m), j=1,2,\cdots, K\\
        \hat{a} &= F(b_1,b_2,\cdots,b_K)
    \end{split}
\end{equation}

We consider a $m\times K$ \LMNet{} as described by system equations (\ref{eq:LMNet:Problem}).
In particular, given a query, we first send it to $m$ independent generators to obtain candidate answers. Next, all answers are sent to $K$ separate selectors, each of which gives a selected answer.
Finally, a fuser aggregates all selected answers to a final output. 

To obtain insights on scaling laws for the above \LMNet{}, we need to model the behavior of each component. In particular, we make the following assumptions. 

\begin{assumption}
The answer space is binary, i.e., $A=\{0,1\}$. All generators are independent and return answer  $1$ with probability $p_G$, i.e.,  $a_i\overset{i.i.d}{\sim} \text{Bernoulli}(p_G)$. All selectors are also independent. Furthermore, each selector follows a two-stage answer generation process. First,  it uses the input candidate answers to update its belief on which answer is better. Next, it generates the selected answer via the updated belief. In particular, let $p_S \in [0,1]$ denote a selector's prior on how likely the right answer is $1$. The selector uses a Bayesian rule to update $p_S$, that is, $\frac{1}{2} (p_S+p_G)$, assuming a beta distribution. Finally, the fuser takes a majority vote approach: it computes the average of all inputs, and return 1 if the average is larger than $1/2$ and 0 otherwise.
\end{assumption}


\subsection{Analysis}
Let us start with an asymptotic analysis: Does the \LMNet{}'s performance continuously improve as the number of selectors and generators go to infinity? Surprisingly, the following theorem gives a negative answer.

\begin{theorem}
    Suppose XXX. If $p_G + p_S >1$, then $m,k\rightarrow \infty$ implies that $Pr[a^*=\hat{a}] \rightarrow 1$. On the other hand, if $p_G + p_S <1$, then $m,k\rightarrow \infty$ implies that $Pr[a^*=\hat{a}] \rightarrow 0$.
\end{theorem}

 
In other words, when the sum of the success rate of the selector and the generator is larger than 1, increasing the number of generators and selectors leads to better response quality. If the sum is smaller than 1, then adding more generators and selectors is only a waste of resources. 
This theorem effectively gives a dichotomy on \LMNet{}'s scaling laws.



\paragraph{Examples.} Suppose $p_G=0.3$ and $p_S=0.8$. Then \LMNet{} with an increasingly large number of selectors and generators gives a correct answer with a large probability. In this case, \LMNet{} is better than querying a generator once. Note that, the standard jury approach~\cite{} is worse than querying a generator once in this case. This is because the selector's quality is higher than a naive voting. Thus, even if the majority of candidate answers are incorrect, we can still find the correct ones. 


Suppose $p_G=0.7$ and $p_S=0.4$. This corresponds to another scenario: the generator is of high quality, but the selector is not. Yet, since there are enough high-quality answers, we can still pick up the high-quality answers. 


Suppose $p_G=p_S=0.4$. This is a hard case. Both generators and selectors are not reliable. In such cases, asking a generator alone is actually better than scaling the \LMNet{}.

\paragraph{Limitation and Next Steps.} First, this is only an asymptotic analysis. Finite-sample analysis is crucial in practice. Second, this modeling assumes a specific form of \LMNet{}. How about other ones potentially with more depths and/or other components? Third, this analysis is based on the simplification of the generation space. How does it generalize to other cases, e.g., the generative settings? Fourth, all generators and selectors are considered homogeneous, but this does not hold in practice. I.e., some generators are better than others. How to take this into account? We can explore these directions in the next few days. 




\newpage
\newpage

\subsection{Building block Modeling}
Let us start by modeling each building block in \LMNet{}.  

Generator: Each generator's answer $\hat{a}_i$ matches the desired answer with probability $p$. 

Judge: Each judge is responsible for generating an answer after reading all generators' answers. Here, let us consider a particular judge form: Bayesian judge. In particular, it encodes all generators' answers as prior knowledge and uses it to update its own generation.

Aggregator: Aggregator gets all information from them.




\begin{equation}
    \hat{a}_i = a \text{ w.p. $p$}
\end{equation}

\begin{equation}
    \sum_{i=1}^{m} \hat{a}_i
\end{equation}


A generator $G_i(\cdot): Q \mapsto A$ takes a query $q\in Q$ as input and generates an answer $a_i\in A$. 


Given a user query and $m$ possible answers from , an answer selector $S_j(\cdot): Q \times A^{m} \mapsto A $ maps 


\subsection{Another modeling}

Capacity v.s. Randomness.



\subsection{Performance Analysis on A \deluxechat{} Instance}
When and why can \deluxechat{} generate answers better than individual generators? We give a formal analysis on a simple instance of \deluxechat{} called $(p_{g,1},p_{g,2},p_s)$ independent \deluxechat{}. 

\begin{definition}
    A \deluxechat{} instance $F$ is called $(p_{g,1},p_{g,2},p_s)$ independent if  
    \begin{itemize}
        \item it has 2 answer generators, $G_1$ and $G_2$,
        \item the two generators and the selector are independent,
        \item generators give  a high-quality answer with probability $p_{g,1},p_{g,2}$ respectively,
        \item selector recognizes the better answer with probability $p_s$.
    \end{itemize}
\end{definition}

Intuitively, $(p_{g,1},p_{g,2},p_s)$ independence focuses on \deluxechat{} with two answer generators. Roughly speaking, the independence assumption ensures that generators are \textit{complementary}, i.e., different LMs perform the best on different user queries. For this \deluxechat{} instance, we can precisely quantify how good the selector must be to ensure $(p_{g,1},p_{g,2},p_s)$ independent \deluxechat{} is better than any individual generator it uses. 


\begin{theorem}\label{thm:deluxechat:selectorquality}
    Suppose $F$ is $(p_{g,1},p_{g,2},p_s)$ independent. Then we have 
    \begin{equation*}
        \Pr[s(\pmb x, F(\pmb x))=1] > \max_{i\in\{1,2\}} \Pr[s(\pmb x, G_i(\pmb x))=1]
    \end{equation*}
    if and only if 
    \begin{equation*}
        p_s >\frac{1}{1+\frac{1-\max_{i}p_{g,i}}{\max_i \frac{p_{g,i}}{p_{g,3-i}}-\max_{i}p_{g,i}}}.
    \end{equation*}
\end{theorem}

There are several implications of Theorem \ref{thm:deluxechat:selectorquality}. First, the quality of the selector plays an important role in \deluxechat{}. In fact,  \deluxechat{}'s performance is better than that of individual generators only when the selector's quality is higher than the threshold given in Theorem \ref{thm:deluxechat:selectorquality}. As a concrete example, suppose two generators are of the same quality ($p_{g,1}=p_{g,2}$). Then the threshold becomes $\frac{1}{2}$, indicating that the selector needs to be better than random guessing. 
Second, the larger gap between the individual generators' quality, the better the selector needs to be. This is because a large quality gap implies a large value of $\max_i{p_{g, i}/p_{g,3-i}}$, and thus a small value of the denominator of the threshold and a large value of the threshold.
These observations suggest that improving (i) the selector quality or (ii) the quality of the relatively weak generator should lead to performance improvement of \deluxechat{} in practice. 


\subsection{Initial Attempts on Scaling Laws}
Now we offer an initial model to study the scaling laws. To do so, we need to first model the generator and the selector in a more fine-grained way.

Generator: $g(\cdot,\cdot)$, where the first parameter encodes the input query, and the second parameter denotes the generation prompt.



Selector: $s(\cdot,\cdot,\cdot)$ The first two are the input answers to compare, and the last is the noise of the selector.


\paragraph{Scaling option 1: adding more selector.}


\newpage
\section{\LMNet{}}
In this section, we introduce and analyze the framework of \LMNet{}. In particular, we would start by defining \LMNet{} formally, then give some common examples of \LMNet{}, and finally analyze and compare the performance of some \LMNet{} instances. 

\subsection{What is \LMNet{}?}
Mathmetically, \LMNet{} is a directed acyclic graph (DAG), where each node is one \LM{}, and each edge indicates how information flows between different \LM{}s. Specifically, an edge pointing to a node represents one input, and an edge pointing out from a node is an output. An node is an \LM{} that transforms (multiple) inputs as (multiple) outputs. Note that a node is determined not only by its inputs, outputs, and \LM{} instances (GPT-4, Claude-2, Llamma, etc), but also its model parameters such as prompts and temperatures.  

\LMNet{} is a generic framework that subsumes many existing concepts and techniques to use. For concreteness, we consider only a few types of nodes in this paper. 

\paragraph{generator.} A generator node is denoted by $g(\cdot,\cdot)$. Here, the first parameter is the input to process, and the second parameter denotes the model parameters,  such as system prompts and temperatures. Intuitively, a generator node is responsible for generating a possible answer to a user query. 


\paragraph{selector.} A selector node is denoted by $s(\cdot,\cdot,\cdot, \cdot)$, where the first parameter represents the user query, the second and third parameters denote two candidate answers, and the last parameter again is the model parameters. The output of a selector is one of the two candidate answers, potentially with some explanations.   %An selector is responsible to select which generation to trust. 

\subsection{\LMNet{} Instances}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figure/InferenceNetwork_flow.pdf}
    \caption{Illustration of the \LMNet{} instances.}
    \label{fig:GPTNet}
\end{figure}
How does a \LMNet{} consisting of only generators and selectors work? While seemingly simple, this has already allowed many interesting \LMNet{} instances.

\paragraph{Warm-up: A two-layer \LMNet{}.} Let us first consider the following simple \LMNet{}.

\begin{align*}
    &r_1 = g(x,\epsilon_1)\\
    &r_2 = g(x,\epsilon_2)\\
    &F_2(x) = s(x, r_1, r_2,\delta)\\
\end{align*}
Here, $x$ is the user query, $\epsilon_1$ and $\epsilon_2$ are the model parameters for the generators, and $\delta$ is the model parameter for the selector.

\paragraph{Selector-scaling \LMNet{}.} Now let us consider a more complicated instance that scaling up the number of selectors. Specifically, it first uses two generators to create two possible answers. Next, it uses two separate selectors to refine the answers, and keep this process for $n$ times. Finally, the output is simply the output from the last selector. This can be formally described by the following equations.  
\begin{align*}
    r_{1,i} &= g(x,\epsilon_{1,i}),i=1,2\\
    r_{k,i} & = s(x, r_{k-1,1}, r_{k-1,2}, \delta_{k,i}), i=1,2, k=2,\cdots, n\\
    F_{s,n}(x) & = r_{n,1}
\end{align*}
Again, $\epsilon_{k,i}$ represent model parameters for the generators, and $\delta_{k,i}$ denote model parameters for the selectors.

\paragraph{Generator-scaling \LMNet{}.} Next let us consider the dual approach to scale up the two-layer \LMNet{}: generator-scaling. In particular, it initializes its answer by querying one generator. 
Next, it updates the answer by (i) generating a new answer, and (ii) comparing it with the current answer by the selector.
This is repeated $n$ times, and then it returns the final answer.  The following system of equations precisely quantifies this \LMNet{}. 

\begin{align*}
    r_1 &= g(x,\epsilon_1)\\
    r'_{k} & = g(x,\epsilon_k), k=2,\cdots, n\\
    r_k & = s(x, r_{k-1}, r_{k}', \delta_k), k=2,\cdots, n\\
    F_{g,n}(x) & = r_n
\end{align*}
Similarly, $\epsilon_{k}$ represent model parameters for the generators, and $\delta_{k}$ denotes model parameters for the selectors.

\subsection{Asymptotic Performance Analysis of \LMNet{}}
Which \LMNet{} should one use? When and why does one \LMNet{} instance outperform another one? Answers to these questions heavily depend on the model parameters for the selectors and the generators. Suppose, for example, the model parameters are always perfect (e.g., they directly encode the correct answer), then the simple two-layer \LMNet{} is sufficient. Therefore, we need to characterize the quality of the model parameters. 

\begin{theorem}
Suppose $\epsilon_1,\epsilon_2$ are iid. And in addition, $\Pr[ q(x,g(x,\epsilon_{1}))=1 ] = p_{g,1}$, $\Pr[ q(x,g(x,\epsilon_{1}))=1 ] = p_{g,2}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=1,q(a_2)=0 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=0,q(a_2)=1 ] = p_{s}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=1,q(a_2)=1 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=0| q(a_1)=0,q(a_2)=0 ] = 1$. W.L.O.G, assume $p_{g,1}\geq p_{g,2}$. Then we have 
    \begin{equation*}
        \Pr[q(\pmb x, F_2(\pmb x))=1] >  \Pr[q(\pmb x, g(\pmb x,\epsilon_1))=1]
    \end{equation*}
    if and only if 
    \begin{equation*}
        p_s >\frac{1}{1+\frac{1-p_{g,1}}{\alpha-p_{g,2}}}.
    \end{equation*}
\end{theorem}
Basically, this says that the two-layer \LMNet{} needs high-quality selector in order to be better than using the better individual generator.

\begin{theorem}
Suppose all model parameters $\epsilon_{k,i}, \delta_{k,i}$ are i.i.d. And in addition, $\Pr[ q(x,g(x,\epsilon_{k,i}))=1 ] = p_{g}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=1,q(a_2)=0 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=0,q(a_2)=1 ] = p_{s}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=1,q(a_2)=1 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=0| q(a_1)=0,q(a_2)=0 ] = 1$. Then we have 
\begin{align*}
   &\Pr[q(x, \lim_{n\mapsto \infty} F_{s,n}(x))=1 ] \\=&p_g^2+ 2p_g (1-p_g) \frac{p_s^2}{p_s^2+(1-p_s)^2}
\end{align*}
\end{theorem}


\begin{theorem}
Suppose all model parameters $\epsilon_{k}, \delta_{k}$ are i.i.d. And in addition, $\Pr[ q(x,g(x,\epsilon_{k}))=1 ] = p_{g}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k}))=1| q(a_1)=1,q(a_2)=0 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=0,q(a_2)=1 ] = p_{s}$, $\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=1| q(a_1)=1,q(a_2)=1 ]=\Pr[ q(x,s(x,a_1,a_2,\epsilon_{k,i}))=0| q(a_1)=0,q(a_2)=0 ] = 1$. Then we have 
\begin{align*}
   &\Pr[q(x, \lim_{n\mapsto \infty} F_{g,n}(x))=1 ] \\=&\frac{p_sp_g}{p_s p_g + (1-p_g)(1-p_s)}
\end{align*}
\end{theorem}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figure/NetCompare.png}
    \caption{Performance differences between the selector network and the generator network.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figure/fitscalelaw.png}
    \caption{Fitting scale laws on the commonsenseqa.}
    \label{fig:enter-label}
\end{figure}

\begin{theorem}[Characterization of network] If $p_g\in\{0,1\}$ or $p_s=\frac{1}{2}$ or $p_s=p_g$, then $\Pr[q(x, \lim_{n\mapsto \infty} F_{s,n}(x))=1 ] = \Pr[q(x, \lim_{n\mapsto \infty} F_{g,n}(x))=1 ]$. If $0<p_g<1, p_s\not=\frac{1}{2}$ and $p_s\not=p_g$, then we have $\Pr[q(x, \lim_{n\mapsto \infty} F_{s,n}(x))=1 ] > \Pr[q(x, \lim_{n\mapsto \infty} F_{g,n}(x))=1 ]$ if and only if $p_g>p_s$.

\end{theorem}
\begin{proof}
    Note that 
    \begin{align*}
   &\Pr[q(x, \lim_{n\mapsto \infty} F_{s,n}(x))=1 ] > \Pr[q(x, \lim_{n\mapsto \infty} F_{g,n}(x))=1 ]
\end{align*}
is equivalent to 
\begin{align*}
   &p_g^2+ 2p_g (1-p_g) \frac{p_s^2}{p_s^2+(1-p_s)^2} > \frac{p_sp_g}{p_s p_g + (1-p_g)(1-p_s)}
\end{align*}
The denominators on both sides are non-negative. Thus, we can multiply both sides by $p_s p_g + (1-p_g)(1-p_s)$ and $p_s^2+(1-p_s)^2$ and obtain 
\begin{align*}
    [p_s p_g + (1-p_g)(1-p_s)][2p_g (1-p_g)p_s^2 +p_g^2(p_s^2+(1-p_s)^2)] > p_s p_g [p_s^2+(1-p_s)^2]
\end{align*}
Let $H(p_s,p_g) \triangleq [p_s p_g + (1-p_g)(1-p_s)][2p_g (1-p_g)p_s^2 +p_g^2(p_s^2+(1-p_s)^2)] - p_s p_g [p_s^2+(1-p_s)^2]$. Thus, 
\begin{align*}
   &\Pr[q(x, \lim_{n\mapsto \infty} F_{s,n}(x))=1 ] > \Pr[q(x, \lim_{n\mapsto \infty} F_{g,n}(x))=1 ]
\end{align*}
if and only if $H(p_s,p_g)>0$. 
Now let us consider $H(p_s,p_g)$. Suppose $p_g>0$. Then we can divide $H(p_s,p_g)$ by $p_g$ to obtain
\begin{align*}
\frac{H(p_s,p_g)}{p_g} = [p_s p_g + (1-p_g)(1-p_s)][2 (1-p_g)p_s^2 +p_g(p_s^2+(1-p_s)^2)] - p_s [p_s^2+(1-p_s)^2]    
\end{align*}
Now, let us view $p_s$ as a constant and $p_g$ as a variable, and then rearrange the terms to obtain 
\begin{align*}
\frac{H(p_s,p_g)}{p_g} & = [p_s p_g + (1-p_g)(1-p_s)][2 (1-p_g)p_s^2 +p_g(p_s^2+(1-p_s)^2)] - p_s [p_s^2+(1-p_s)^2]    \\
&= [(2p_s-1) p_g +(1-p_s)][ p_g(p_s^2+(1-p_s)^2-2p_s^2) + 2 p_s^2] - p_s [p_s^2+(1-p_s)^2] \\
&= [(2p_s-1) p_g +(1-p_s)][ (1-2p_s) p_g + 2 p_s^2] - p_s [p_s^2+(1-p_s)^2]
\end{align*}
Now expanding all terms in the first product gives
\begin{align*}
\frac{H(p_s,p_g)}{p_g} 
&= [(2p_s-1) p_g +(1-p_s)][ (1-2p_s) p_g + 2 p_s^2] - p_s [p_s^2+(1-p_s)^2] \\
&= -(1-2p_s)^2 p_g^2 +  [(2p_s-1)2p_s^2+(1-2p_s)(1-p_s)] p_g + (1-p_s) 2p_s^2 - p_s [p_s^2+(1-p_s)^2]
\end{align*}
Now we can rewrite this equality as 
\begin{align*}
\frac{H(p_s,p_g)}{p_g} 
&= -(1-2p_s)^2 p_g^2 +  [(2p_s-1)2p_s^2+(1-2p_s)(1-p_s)] p_g + (1-p_s) 2p_s^2 - p_s [p_s^2+(1-p_s)^2]\\
&=  -(1-2p_s)^2 p_g^2 +  (1-2p_s)(1-p_s-2p_s^2) p_g - p_s [p_s^2+(1-p_s)^2-2p_s(1-p_s)]\\
&=  -(1-2p_s)^2 p_g^2 +  (1-2p_s)(1-p_s-2p_s^2) p_g - p_s (1-2p_s)^2\\
&= -(1-2p_s) [(1-2p_s)p_g^2 - (1-p_s-2p_s^2) p_g +p_s (1-2p_s)]\\
&= -(1-2p_s) [(1-2p_s)p_g^2 - (1-2p_s)(1+p_s) p_g +p_s (1-2p_s)]\\
&= -(1-2p_s)^2  
[p_g^2-(1+p_s)p_g+p_s]\\
&= -(1-2p_s)^2  (p_g-p_s)(p_g-1)
\end{align*}
Here, the second equality is by expanding all terms, the third equality is by algebraic rewriting the third term from the last equation, the fourth equation extracts the common factor $1-2p_s$, the fifth equation uses the fact that $1-a-2a^2=(1+a)(1-2a)$, the sixth equation extract the common factor $1-2p_s$ again, and the final equation uses the fact that $a^2-(1+b)a+b=(a-b)(a-1)$.
Therefore, we have shown that 
\begin{align*}
    H(p_s,p_g) = - p_g (1-2p_s)^2 (p_g-p_s) (p_g-1)
\end{align*}
$H(p_s,p_g)>0$ if and only if $0<p_g<1,p_s\not=\frac{1}{2}, p_g >p_s$. 
\end{proof}

\subsection{Finite sample analysis}
How does the performance scale as a function of the number of generators and selectors? At least we can have a simulation-based analysis.

Selector Net: 

\begin{align*}
    q(F_{s,n}(x)) = [1,\frac{1}{2}, 0] S^n\begin{pmatrix}
        p_g^2\\
        2p_g(1-p_g)\\
        (1-p_g)^2\\
    \end{pmatrix} 
\end{align*}

Generator Net:
\begin{align*}
    q(F_{g,n}(x)) = [1,0]\left[G^n \begin{pmatrix}
        p_g\\
        1-p_g
    \end{pmatrix}\right]
\end{align*}
where
\begin{align*}
G = \begin{pmatrix}
p_g + (1 - p_g) p_s & p_g p_s \\
(1 - p_g) (1 - p_s) & 1 - p_s p_g
\end{pmatrix}
\end{align*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/finite_analysis.pdf}
    \caption{Finite sample analysis on the generator and selector net.}
    \label{fig:enter-label}
\end{figure}
\subsection{modeling selectors with multiple inputs}
The selector quality depends on two factors, (i) $n$ the number of inputs, and (ii) $r$ the fraction of correct answers.

The probability of getting a correct answer is 
\begin{align}
    p_{n,r} = \alpha(n) +r^{\beta(n)} (1-\alpha(n))
\end{align}
where 
\begin{align}
    \alpha(n) = \exp(-(n-z)^2)
\end{align}
and 
\begin{align}
    \beta(n) = \exp(-\gamma n)
\end{align}


Another simplified model is 
\begin{align*}
    P_{n,r} = [(1-c) r + c]^{a \log n +b }
\end{align*}
\subsection{Some research questions to answer}
\begin{itemize}
    \item How do these analytical models match the empirical results?
    \item How to connect the hierarchical scaling with multiple-input selector's scaling?
    \item How do we justify the multiple-input selector' model?
    \item How to extend the asymptotic analysis to finite sample analysis? 
\end{itemize}


\section{An analytical model to explain the U shape}
By contrast to the traditional wisdom on scaling laws of training data and model parameters, the experiments shown in Figure \ref{} suggest that \LMNet{}'s performance is not necessarily monotone w.r.t. the number of network components. Why is this the case? In this section, we offer an analytical model to explain this phenomenon. The key insight is that, in a nutshell, the data matters.


\subsection{System models}
Let us consider a simple network: given a query $x$, we generate $K$ candidate answers $z_1, z_2, \cdots, z_K$, and then take the majority vote as the final response. Suppose all $z_i$ are generated independently from some population, and let $p_x$ be the probability of the answer being correct. Let $f(x;k)$ denote the probability of the final answer being correct and let us denote the log-likelihood $F(k;D) \triangleq \mathbb{E}_{x\sim D} [\log f(x;k)]$ as the loss function. 
As a first step, let us consider binary prediction tasks, and when it is clear from the context, let us 

Now our question is, How does $F(k;D)$ scale as a function of $k$?

\subsection{Scaling laws for a fixed $x$}
Let us start by considering how $f(x;k)$ scales. W.L.O.G, suppose the correct answer is $1$, and then the majority vote network is correct when 
\begin{align*}
    \frac{1}{K}\sum_{K}^{i=1}z_i > \frac{1}{2}
\end{align*}
Noting that $z_i$ is correct with probability $p_x$, we can rewrite the above as 

\begin{align*}
    \frac{1}{K}\sum_{K}^{i=1}z_i - p_x > \frac{1}{2} - p_x
\end{align*}

Suppose $p_x>\frac{1}{2}$. The above event implies $|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| < p_x - \frac{1}{2}$. Applying 
Hoeffding's inequality gives that 
\begin{align*}
\Pr[|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| < p_x - \frac{1}{2}] \geq 1-2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}
Thus, we have 
\begin{align*}
    f(x;k) = \Pr[\frac{1}{K}\sum_{K}^{i=1}z_i>\frac{1}{2}] \geq  1 - 2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}

Suppose $p_x<\frac{1}{2}$. Then the above event implies $|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| > \frac{1}{2}-p_x$. Now applying Hoeffding's inequality gives us that 
\begin{align*}
\Pr[|\frac{1}{K}\sum_{K}^{i=1}z_i - p_x| > 1/2- p_x ] \leq 2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}
That is, 
\begin{align*}
    f(x;k) = \Pr[\frac{1}{K}\sum_{K}^{i=1}z_i>\frac{1}{2}] \leq  2 \exp(-\frac{2(p_x-1/2)^2}{K})
\end{align*}
To sum up, we have the following result
\begin{align*}
    f(x;k) \begin{cases}
        \geq   1 - 2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x >\frac{1}{2}\\
        \leq 2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x < \frac{1}{2}
    \end{cases}
\end{align*}

For large $K$, Hoeffding's inequality is ``tight'', and thus we can approximate the above inequalities by equality and obtain 

\begin{align*}
    f(x;k) \approx g(x;k) \triangleq \begin{cases}
        1 - 2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x >\frac{1}{2}\\
         2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x < \frac{1}{2}
    \end{cases}
\end{align*}
This gives a scaling law that depends on the given problem: if the problem is easy, i.e., most samples are correct ($p_x > \frac{1}{2}$), then generating more candidate answers improves the performance. if the problem is hard, i.e., most samples are incorrect ($p_x < \frac{1}{2}$), adding more candidate answers lowers the performance!

\subsection{Scaling laws for $F(k;D)$}
The previous section suggests that for fixed query $x$,  enlarging the network monotonically improves or worsens the performance, depending on the difficulty of the query $x$. In practice, the problem difficulty is diverse. Therefore, there is a balance between easy and hard problems: easy problems need more candidate answers, but hard problems want fewer. This intuitively explains why empirically the scaling performance is non-monotone. 

Now let us make the above intuition formal by quantifying the loss function. This is, of course, intractable for general data distribution $D$. For simplicity, let us consider a simple instance $D(p_1, p_2, \alpha)$. Here, the data distribution is a mixture of two distributions. All problems in the first is easy with correct probability $p_x=p_1>\frac{1}{2}$. And the second distribution contains hard problems, where each candidate answer is correct with probability $p_x=p_2<\frac{1}{2}$. $\alpha$ is the fraction of samples from the first distribution. Now let us expand $F(K;D)$ as
\begin{align*}
    F(K;D) = &\mathbb{E}_{x\sim D} \log f(x;K) \approx G(K;D) = \mathbb{E}_{x\sim D} \log g(x;K) \\
    =& \alpha \log  [1-2 \exp(-\frac{2(p_1-1/2)^2}{K})]  + (1-\alpha)\log[2 \exp(-\frac{2(p_2-1/2)^2}{K}]) \\
    = & \alpha \log  [1-2 \exp(-\frac{2(p_1-1/2)^2}{K})]  - \frac{2(1-\alpha)(p_2-1/2)^2}{K} + (1-\alpha) \log 2\\
\end{align*}

This is the scaling law of the loss as a function of the number of candidate answers for distribution $D(p_1,p_2,\alpha)$. 
While simple, this also sheds light on scaling laws for general distributions $D$. In fact, one can approximate any distribution $D$ by discretizing the value of an candidate answer being correct, and in general, we can make this an integral. 

\subsection{Optimal candidate answer size}
What is the optimal candidate answer size? Let us keep studying the above distribution instance. By COV, let $M\triangleq\frac{1}{K}$, we can rewrite it as  

\begin{align*}
    G(1/M;D) 
    = & \alpha \log  [1-2 \exp(-2(p_1-1/2)^2M)]  - 2(1-\alpha)(p_2-1/2)^2M + (1-\alpha) \log 2\\
\end{align*}
The first term is concave, the second term is linear in $M$, and hence the above is concave in $G$. Therefore, any stationary points are optimal. Let us take the derivative 

\begin{align*}
    \partial \frac{G(1/M;D)}{\partial M} 
    = & \alpha \frac{-4(p_1-1/2)^2 \exp(-2(p_1-1/2)^2M)}{1-2 \exp(-2(p_1-1/2)^2M)}   - 2(1-\alpha)(p_2-1/2)^2\\
\end{align*}
Let $W = \exp(-2(p_1-1/2)^2M)$.
Then above is 
\begin{align*}
    \partial \frac{G(1/M;D)}{\partial M} 
    = & \alpha \frac{4(p_1-1/2)^2 W)}{1-2 W}   - 2(1-\alpha)(p_2-1/2)^2\\
\end{align*}
$ \frac{\partial G(1/M;D)}{\partial M} =0$ implies 

\begin{align*}
    W = \frac{c_2}{\alpha c_1+2 c_2}
\end{align*}
where $c_1 = 4(p_1-1/2)^2$ and $c_2 = 2(1-\alpha) (p_2-1/2)^2$.

Now map $W$ back to $K$ we have
\begin{align*}
    K^* = \frac{-2(p_1-1)^2}{\log \frac{c_2}{\alpha c_1 +2 c_2}}
\end{align*}

Note that, interestingly, the solution is unique and positive. It is not hard to prove that, $G(K;D)$ increases until $K=K^*$ and then it decreases. This matches the empirical observations.  

\subsection{Fitting the scaling laws }
There are many ways to fit the scaling laws for a real-world problem. here we list two of them.

\paragraph{Problem Difficulty Estimation.} The key observation of the non-monotone scaling comes from problem difficulty heterogeneity. Thus, a natural idea is to estimate the problem's difficulty first and then plug in the values $p_1, p_2$ in the scaling laws. More generally, as we mentioned before, one can use other parametric versions of the data hardness to fit this. 

\paragraph{Direct estimation Formula fitting.} Note that our goal is to predict $F(K;D)$ while all analysis is assume $F(K;D)\approx G(K;D)$. That is to say, even if the difficulty estimation is perfect, the plugging-in approach may not be accurate as well. Thus, an alternative approach is to directly estimate the parameters in the scaling law.
Recall that the scaling law is
\begin{align*}
    G(K;D)
    = & \alpha \log  [1-2 \exp(-\frac{2(p_1-1/2)^2}{K})]  - \frac{2(1-\alpha)(p_2-1/2)^2}{K} + (1-\alpha) \log 2\\
\end{align*}
And W.L.O.G, we can simply rewrite it as 
\begin{align*}
    G(K;D)
    = & c_1  \log  [1-c_2 \exp(-\frac{c_3}{K})]  - \frac{c_3}{K} + c_4\\
\end{align*}
Now, we can use training data to fit the constant $c_1,c_2,c_3,c_4$, and then directly predict the scaling law. One benefit here is that, this can hopefully mitigate the approximation error $F(K;D)-G(K;D)$ 

\subsection{What experiments to run?}
We need to verify this asusmp

TODO: cleaning the remaining. 
\newpage

\subsection{Building Blocks}

Generator: $g(\cdot,\cdot)$, where the first parameter encodes the input query, and the second parameter denotes the generation prompt.



Selector: $s(\cdot,\cdot,\cdot,\cdot)$. The first is the input query,  The second two are the two candidate answers to compare, and the last is the selector prompt.


\subsection{The Two layer \LMNet{}: A warm-up}
Let us consider a warm-up example. 



\subsection{Scaling up the selectors}
\begin{align*}
    r_{1,i} &= g(x,\epsilon_{1,i}),i=1,2\\
    r_{k,i} & = s(x, r_{k-1,1}, r_{k-1,2}, \delta_{k,i}), i=1,2\\
    \hat{r} & = r_{n,1}
\end{align*}


\subsection{Scaling up the generators}


\begin{align*}
    r_1 &= g(x,\epsilon_1)\\
    r'_{k} & = g(x,\epsilon_k)\\
    r_k & = s(x, r_{k-1}, r_{k}', \delta_k)\\
    \hat{r} & = r_n
\end{align*}

How do we measure the quality? 

\begin{align*}
    \Pr[q(\hat{r},x)=1]
\end{align*}


Assumptions:
\begin{itemize}
    \item $\epsilon, \delta$ are i.i.d.
    \item $\Pr[]$
\end{itemize}


\begin{theorem}
    $\Pr[q(r_s)=1] = p_g^2+2p_g(1-p_g) \frac{p_s^2}{p_s^2+(1-p_s)^2}$
\end{theorem}
\subsection{}


We are showing paradigm that leverages the knowledge of the

Now we have a qualitative understanding of the scaling properties, but how about the quantitative analysis? In principle, the performance formula of $F(D;K)$ is sufficient, but it is still hard to tell exactly the performance from there.  Here, we study how the function $F(D;K)$ may be approximated using a simple form. 
Suppose $p_x>1/2$, the probability of being correct $f(x;K)$ is $f(x;K) = 1- \Pr\left[\sum^{K}_{i=1}z_i \leq \frac{K}{2}\right]$.  

\begin{align*}
    f(x;k) \approx g(x;k) \triangleq \begin{cases}
        1 - 2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x >\frac{1}{2}\\
         2 \exp(-\frac{2(p_x-1/2)^2}{K}), & p_x < \frac{1}{2}
    \end{cases}
\end{align*}
Therefore, the overall performance is 
\begin{align*}
    F(D;K) = G(D;K) = \alpha (1-\exp(-2K(p_1-1/2)^2)) + (1-\alpha) \exp(-2K(p_2-1/2)^2))
\end{align*}
The optimal sample size is 

\begin{align*}
    \hat{K} = \frac{\log [\alpha/(1-\alpha) (p_1-1/2)^2/(p_2-1/2)^2]}{(p_1-1/2)^2-(p_2-1/2)^2}
\end{align*}


\subsection{Fitting the Scaling Laws in Practice}
How do we fit the scaling laws on real-world tasks?  
\paragraph{Problem Difficulty Estimation.} The key observation of the non-monotone scaling comes from problem difficulty heterogeneity. Thus, a natural idea is to estimate the problem's difficulty first and then plug in the values $p_1, p_2$ in the scaling laws. More generally, as we mentioned before, one can use other parametric versions of the data hardness to fit this. 

\paragraph{Direct estimation Formula fitting.} Note that our goal is to predict $F(K;D)$ while all analysis is assume $F(K;D)\approx G(K;D)$. That is to say, even if the difficulty estimation is perfect, the plugging-in approach may not be accurate as well. Thus, an alternative approach is to directly estimate the parameters in the scaling law.
We can simply rewrite it as 
\begin{align*}
    G(K;D)
    = & c_1 \exp^{-b_1 K} - c_2 \exp^{-b_2 K} + c_3
\end{align*}
Now, we can use training data to fit the constant $c_1,c_2,c_3,b_1, b_2$, and then directly predict the scaling law. One benefit here is that, this can hopefully mitigate the approximation error $F(K;D)-G(K;D)$ 

\begin{align*}
    \min_{c,b} \ell (G(K;D) - F(K;D))
\end{align*}
\begin{align*}
\boxed{a}    
\end{align*}

Naively applying the above on small $K$ gives poor performance on large $K$. 

\paragraph{A two-stage process.}

First, estimate $\alpha$ using a few samples. 

Second, estimate $F_1(K)$ by $G_1(K) = 1 - \exp(-a_1 K - a_2 \sqrt{K} + a_3) $


Third, estimate $F_2(K)$ by $G_2(K) = \exp(-b_1 K - b_2 \sqrt{K} + b_2)$







Performance Prediction for Generic Datasets and Tasks
So far, our analysis has focused on data distribution with a $2$-level difficulty and tasks with answer space size $\|A\|=2$. Now we show a generalization to generic data and tasks. 

\paragraph{Generalization to generic data distribution.} By definition, the performance on a generic data with difficulty distribution $\mathcal{P}$ is $F(K;D) = \mathbbm{E} [y=\hat{y}] = \mathbbm{E}[\mathbbm{E}[y=\hat{y}|r(x)=p] \cdot \mathbbm{1}_{r(x)=p}] = \mathbbm{E}[ I_p(\frac{K+1}{2},\frac{K+1}{2}) \cdot \mathbbm{1}_{r(x)=p}]$. Let $p(\cdot)$ denote the pdf (or pmf) of $r(x)$. We can rewrite this as  $F(K;D) = \int_{0}^{1} I_t(\frac{K+1}{2},\frac{K+1}{2}) p(t) dt$. It is challenging to precisely characterize how the difficulty distribution $\mathcal{P}$ affects the performance landscape and optimal network sizes due to the integral. However, one can still show that there exists some difficulty distribution $\mathcal{P}$, such that the shape of the performance landscape can be monotone, a U-shape, or even zig-zag. This further highlights the importance of carefully choosing the network sizes. 

\paragraph{Generalization to tasks with answer space size $\|A\|>2$.} A precise analysis for generic tasks is even more challenging, as there is no closed form for the performance on an individual item with difficulty $p$. Fortunately, we can give an upper and lower bound on it. To see this, simply note, among all candidate answers, (i) that if the fraction of correct answers is larger than $\frac{1}{2}$, then the correct answer must be choices of majority vote, and (ii) that if the correct answer is the majority vote, then at least $\frac{1}{\|A\|}$ fraction of answers must be correct. This gives the inequality 
$
\Pr\left[\frac{1}{K}\sum^{K}_{i=1}\mathbbm{1}_{z_i =y}> \frac{1}{d}\right]   \geq  \mathbbm{E}[{y=\hat{y}}] \geq  \Pr\left[\frac{1}{K}\sum^{K}_{i=1}\mathbbm{1}_[z_i=y] > \frac{1}{2}\right]
$. Thus, aggregating both sizes over the difficulty distributions gives an upper and lower bound on the overall performance on a generic distribution $D$ with arbitrary answer space size.

What does the above analysis imply in practice? One important observation is that we can predict \LMNet{} performance on generic data with arbitrary answer space. To see this, notice that the upper and lower bounds can both be approximated by the function $g(K;a_1, a_2, a_3)$ with varying parameters $a_1, a_2, a_3$. Thus, for each item, we can directly fit $a_1, a_2, a_3$ to estimate the performance, and then aggregate over all items in a training dataset. We give the details in Algorithm \ref{alg:ScaleLaw:Estimation}. 
%\james{Some of the notations below are not consistent with above (e.g. $F_x(t)$) and can be simplified}

\begin{algorithm}
\caption{Scaling Law Estimation}\label{alg:ScaleLaw:Estimation}
\KwIn{A training dataset $D_{Tr}=\{x_i, y_i, \{z_{i,m}\}_{k=1}^{K},\{F(t;\{x_i\})\}_{t\in T}^{}\}_{i=1}^{n}$ }
\KwOut{The scaling function $G(K)$}
\For{$i=1$ \KwTo $n$}{
    
    $\hat{y}_i = \arg\max_{a\in A} \sum_{m=1}^{M}\mathbbm{1}_{z_{i,j} = a} $ \tcp{Identify majority choices}
    $G_i(K;\alpha) = \begin{cases}
    \frac{1 - \exp(-a_1 K  -a_2 K^{1/2}-a_3 )}{\|\hat{Y}_i\|}, & \textit{$ y_i = \hat{y}_i $ } \\
        \exp(-a_1 K  -a_2 K^{1/2}-a_3 ), & o/w        
    \end{cases}$\tcp{choose the parametric form}

    Obtain $\pmb c_i = \arg\min_{\alpha} \sum_{t\in T}^{} \ell(G_i(t;\alpha), F(t;\{x_i\}))$
    
}
Return $G(K) = \frac{1}{n}\sum_{i =1}^{n} G_i(K;\pmb c_i)$
\end{algorithm}



It is not hard to show that as $a$ increases, the incomplete beta function $I_x(a,a)$ monotonically increase/decrease if $x>\frac{1}{2}$ ($x<\frac{1}{2}$). That is, more LM calls lead to better performance on easy queries ($d_V(x)<0$) but worse performance on difficult ones ($d_V(x)>0$). performance $F(K,x)$ 
This shows different scaling trends for difficult and easy queries. In fact, since the incomplete beta function $F(K,x)$ monotonically increases  $d_V(x)>0$


Let us first break down the performance on difficult and easy queries, i.e.,  $F(K,D) = E_{x\sim D}[F(K,x)|d(x)>0]\Pr[d(x)>0] + E_{x\sim D}[F(K,x)|d(x)<0]\Pr[d(x)<0]$.


We can first give To see how it works, 

For difficult query $x$, $F(K,x)$ should follow a negative exponential law, while for easy query $x$ it should follow  

$F(K,D) = E_{x\sim D}[\hat{y}_K(x)=y|d(x)>0]\Pr[d(x)>0] + E_{x\sim D}[\hat{y}_K(x)=y|d(x)<0]\Pr[d(x)<0]$



Now we analyze Voting \LMNets{} with a focus on their scaling properties. In particular, we (i) characterize how \dataitem{}  difficulty shapes the performance landscape, (ii) derive the optimal number of LM calls as a function of the \dataitem{}  difficulty,  
(iii) propose a scaling law, and (iv) present an algorithmic paradigm to estimate the scaling law parameters using a small number of samples. For ease of reference, we have listed all major notations in Table \ref{tab:ScaleLaw:Notations}.



\subsection{Item  Difficulty}
How can we quantify the difficulty of a query item $x$ in an evaluation task? One natural option is  \textit{correct answer rate}, i.e., how likely a candidate answer is correct,  denoted by $r(x) \triangleq \mathbb{E}_{\theta \sim \Theta} [G(x,\theta) =y]\in [0,1]$.
Intuitively, large $r(x)$ indicates that the query $x$ is relatively easy to answer, and small $r(x)$ implies that it is hard. If $r(x)>0.5$, we call  $x$ an ``easy'' query. Otherwise, we call it a ``hard'' query.

Now, we can quantify the difficulty of a data distribution $D$ by a distribution over the item difficulty, denoted by $\mathcal{P}$. That is, for an item $x$ randomly drawn from  $D$, its difficulty $r(x)$ follows   $\mathcal{P}$.

{\color{red} TODO. }

\subsection{Problem Statement}
Our goal is to study the \textit{scaling properties of one-layer Voting \LMNets{}}, i.e., how the number of LM calls $K$ affects an \LMNet{}'s performance on a data distribution $D$, denoted by $F(K;D)$. For exposure purposes, we focus on the expected $0/1$ loss as the performance metric, i.e.,
$F(K;D) = \mathbbm{E}[\hat{y}=y]$, where the expectation is taken over the data distribution $D$ and the sample parameters $\theta_1,\theta_2, \cdots, \theta_K$ in the Voting \LMNet{}. 
Note that our analysis can generalize to other loss functions as well. For simplicity, let us also assume that the difficulty of items in $D$ takes values from only two values. More specifically, for a query $x\in D$,
\begin{align*}
r(x) = \begin{cases}
    p_1, & \textit{ with probability } \alpha \\
    p_2, & \textit{ with probability } 1-\alpha \\
\end{cases}    
\end{align*}
We say that such a $D$ is \textit{$2$-level difficult} with parameter $(\alpha, p_1, p_2)$. W.L.O.G, let us assume $p_1> p_2$.  We also suppose that the answer space $A$ contains only two possible answers.
We will discuss how some of our results can be generalized to the generic difficulty distribution and answer space, but we leave an in-depth as future work.


\subsection{\Dataitem{}  Difficulty Shapes Performance Landscape}
\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figure/method/InferenceNetwork_shape.pdf}
    \caption{How the \dataitem{} difficulties shape the landscape of a one-layer Voting \LMNet{}'s performance. Informally, if the overall task is ``easy'' ($p_1+p_2>1$), but the fraction of ``hard'' queries is large ($\alpha<1-\frac{1}{t}$), then as the number of LM calls increases, the Voting \LMNets{}' performance increases first but then decreases. We call such a landscape a ``inverse U shape''. 
Similarly,  if the overall task is ``hard'' ($p_1+p_2<1$), but the fraction of ``hard'' queries is small ($\alpha>1-\frac{1}{t}$), then enlarging the number of LM calls leads an initial decrease and then increase. Such a landscape is called a ``U shape''. When $\alpha$ is large, the U-shape is less likely to occur while the inverse U-shape becomes more common. Smaller $\alpha$ leads to an opposite trend.}
    \label{fig:ScaleLaw:Landscape}
\end{figure}
How does the \dataitem{} difficulty affect the performance landscape of a one-layer Voting \LMNet{}? The following theorem gives a qualitative characterization. %how the difficulty parameters $(\alpha, p_1, p_2)$ affect the performance landscape. 
 %To answer this, let us first connect \LMNet{}'s performance with data difficulty via the lens of incomplete beta function. 

%Here, the two terms correspond to the performance on queries with difficulty $p_1$ and $p_2$ respectively. It is easy to see that the performance is monotonically increasing (or decreasing) if both $p_1,p_2$ are larger (or smaller) than $\frac{1}{2}$. It becomes interesting when $p_1>\frac{1}{2}$ and $p_2<\frac{1}{2}$: as $K$ increases, the first incomplete beta function becomes larger, but the second incomplete beta function gets smaller. The following theorem qualitatively characterizes how the difficulty parameters $(\alpha, p_1, p_2)$ affect the performance landscape. 

%\james{If there are three or more levels of difficulty, can the curve have multiple ups and downs?}

\begin{theorem}\label{thm:scaleLaw:character}
Suppose $D$ is $2$-level difficult with $(\alpha, p_1,p_2)$,  $\|A\|=2$, and $K$ is odd W.L.O.G. Let $t\triangleq \frac{p_2 (1-p_2) (\frac{1}{2}-p_2)}{p_1 (1-p_1) (p_1-\frac{1}{2})}+1$. If  $p_1+p_2\not=1$ and $p_2<\frac{1}{2}<p_1$, then as $K$ increases, $F(K;D)$ 
   \begin{itemize}
       \item  increases monotonically, if $p_1+p_2>1$ and  $\alpha \geq 1-\frac{1}{t}$
       \item decreases monotonically,  if $p_1+p_2<1$ or $\alpha\leq 1-\frac{1}{t}$
       \item increases and then decreases, if $p_1+p_2>1$ and $\alpha<1-\frac{1}{t}$
       \item decreases and then increases, if $p_1+p_2<1$ and $\alpha>1-\frac{1}{t}$
   \end{itemize}
   \end{theorem}

Theorem \ref{thm:scaleLaw:character} precisely connects the \dataitem{} difficulty with the performance landscape. Here, $t$ is a constant that only depends on $p_1$ and $p_2$, i.e., the probability of an LM's generation being correct on easy and hard queries, respectively. Intuitively, $t$ quantifies the difficulty similarity between the easy and hard queries: it becomes larger if the easy queries are more difficult ($p_1$ is smaller) or the hard queries are less difficult ($p_2$ is larger).  Interestingly, it suggests that, for some \dataitem{} difficulty distribution, a non-monotone effect of the number of LM calls is expected. Informally, if the overall task is ``easy'' ($p_1+p_2>1$), but the fraction of ``hard'' queries is large ($\alpha<1-\frac{1}{t}$), then as the number of LM calls increases, the Voting \LMNets{}' performance increases first but then decreases. We call such a landscape a ``inverse U shape''. 
Similarly,  if the overall task is ``hard'' ($p_1+p_2<1$), but the fraction of ``hard'' queries is small ($\alpha>1-\frac{1}{t}$), then enlarging the number of LM calls leads an initial decrease and then increase. Such a landscape is called a ``U shape''. 
This well explains the U-shape of \LMNets{}' performance shown in Figure \ref{fig:ScaleLaw:intro1}.Figure \ref{fig:ScaleLaw:Landscape} visualizes the effects of \dataitem{} difficulty on the performance landscape in more detail. 

\subsection{\Dataitem{} Difficulty Determines Optimal Number of LM Calls}
We have shown that there are cases where, determined by \dataitem{} difficulty distribution,   a non-monotone scaling behavior of Voting \LMNets{} is expected.  In these cases, blindly scaling up the number of LM calls may not lead to the desired performance. 
How should one determine the number of LM calls in these cases? The following result gives a precise answer.

\begin{theorem}\label{thm:scalelaw:optimalnetworksize}
Suppose $D$ is $2$-level difficult with $(\alpha, p_1,p_2)$, $\|A\|=2$, and $K$ is odd W.L.O.G. If $p_1+p_2>1$ and $\alpha<1-\frac{1}{t}$, then the number of LM calls  $K^*$ that maximizes the overall performance of an one-layer Voting \LMNet{}(up to rounding) is 
\begin{align*}
    K^* = 2 \frac{\log\frac{\alpha}{1-\alpha}\frac{2p_1-1}{1-2p_2}}{\log \frac{p_2(1-p_2)}{p_1(1-p_1)}} 
\end{align*}
\end{theorem}
As expected, the optimal number of LM calls depends on the \dataitem{} difficulty. For example, $K^*$ will be larger if $\alpha$ grows (up to $1-\frac{1}{t}$). 
That is, if there are more ``easy'' queries than ``hard'' queries, then a larger network should be adopted. This suggests that a difficulty-aware design of Voting \LMNets{} may offer better performance than a difficulty-agnostic design. We will analyze $K^*$ in detail in Section \ref{sec:scalelaw:exp_optimalsize}. 


\subsection{A Scaling Law for One-layer Voting \LMNets{}}
We have seen that inference system performance is closely related to item difficulty. 
What is an intuitive way to explicitly model \dataitem{} difficulty in a scaling law of Voting \LMNets{}? 
Here, we propose the following function $G(\cdot;\cdot)$ 
 as a scaling law on the dataset $D$ with 2-level difficulty 
\begin{align*}
G(K;D) \triangleq \alpha g_{p_1}(K;\pmb c_1) + (1-\alpha) g_{p_2}(K;\pmb c_2)   
\end{align*}
where 
\begin{align*}
    g_p(K;\pmb c) \triangleq \begin{cases}
       1 - \exp(- \pmb c^T [K,\sqrt{K},1]) & \textit{if } p> \frac{1}{2}\\
       \exp(- \pmb c^T [K,\sqrt{K},1])  &  \textit{if } p< \frac{1}{2} \\
    \end{cases}
\end{align*}
This scaling law encodes how the \dataitem{} difficulty affects the performance. For example, if  $p_1>\frac{1}{2}$ and $p_2<\frac{1}{2}$, the first term $g_{p_1}(\cdot;\cdot)$ will monotonically increase while the second term $g_{p_2}(\cdot;\cdot)$ will  monotonically decrease, and hence the overall scaling function $G(K;D)$ exhibits a non-monotone behavior. This also captures that the number of LM calls changes the performance at an exponential rate.

This scaling law can be easily generalized to data $D$ with generic \dataitem{} difficulty distribution. In particular, if the density function of the \dataitem{} difficulty is $q(u)$, then we can generalize the scaling law for the 2-level difficulty to this case via 
\begin{align*}
G(K;D) \triangleq \int_{0}^{1}  g_{q(u)}(K;\pmb c_u) q(u) d u     
\end{align*}
For discrete distribution, one can simply replace the integral by summation and the density function by the mass function.

\subsection{Estimating the Scaling Law Parameters}
In practice, an important problem is to learn the scaling law using a small number of samples. Here, we give an algorithmic paradigm to estimate the scaling law parameters and thus the overall scaling function $G(\cdot;\cdot)$, as shown in Algorithm \ref{alg:ScaleLaw:Estimation}.

The estimation paradigm contains two major steps: it first estimates the scaling parameter for each item in the training dataset, and then aggregates the results to obtain the overall scaling function. To estimate the scaling law on each item, it first compares the majority vote on a few samples (line 2) with the true label to determine if the query is easy or not and thus selects the parametric form (line 3). Then it uses the empirically observed performance on a few samples to fit the parameters (line 4). For demonstration purposes, we use a square loss function as the optimization metric. %\james{explain what loss function we use for estimation in step 4.}. 
Finally, the aggregation (line 5) over each item's scaling function is returned as the final estimation.


\eat{\paragraph{Generalization to generic data distribution.} By definition, the performance on a generic data with difficulty distribution $\mathcal{P}$ is $F(K;D) = \mathbbm{E} [y=\hat{y}] = \mathbbm{E}[\mathbbm{E}[y=\hat{y}|r(x)=p] \cdot \mathbbm{1}_{r(x)=p}] = \mathbbm{E}[ I_p(\frac{K+1}{2},\frac{K+1}{2}) \cdot \mathbbm{1}_{r(x)=p}]$. Let $p(\cdot)$ denote the pdf (or pmf) of $r(x)$. We can rewrite this as  $F(K;D) = \int_{0}^{1} I_t(\frac{K+1}{2},\frac{K+1}{2}) p(t) dt$. It is challenging to precisely characterize how the difficulty distribution $\mathcal{P}$ affects the performance landscape and optimal network sizes due to the integral. However, one can still show that there exists some difficulty distribution $\mathcal{P}$, such that the shape of the performance landscape can be monotone, a U-shape, or even zig-zag. This further highlights the importance of carefully choosing the network sizes. 

\paragraph{Generalization to tasks with answer space size $\|A\|>2$.} A precise analysis for generic tasks is even more challenging, as there is no closed form for the performance on an individual item with difficulty $p$. Fortunately, we can give an upper and lower bound on it. To see this, simply note, among all candidate answers, (i) that if the fraction of correct answers is larger than $\frac{1}{2}$, then the correct answer must be choices of majority vote, and (ii) that if the correct answer is the majority vote, then at least $\frac{1}{\|A\|}$ fraction of answers must be correct. This gives the inequality 
$
\Pr\left[\frac{1}{K}\sum^{K}_{i=1}\mathbbm{1}_{z_i =y}> \frac{1}{d}\right]   \geq  \mathbbm{E}[{y=\hat{y}}] \geq  \Pr\left[\frac{1}{K}\sum^{K}_{i=1}\mathbbm{1}_[z_i=y] > \frac{1}{2}\right]
$. Thus, aggregating both sizes over the difficulty distributions gives an upper and lower bound on the overall performance on a generic distribution $D$ with arbitrary answer space size.

What does the above analysis imply in practice? One important observation is that we can predict \LMNet{} performance on generic data with arbitrary answer space. To see this, notice that the upper and lower bounds can both be approximated by the function $g(K;a_1, a_2, a_3)$ with varying parameters $a_1, a_2, a_3$. Thus, for each item, we can directly fit $a_1, a_2, a_3$ to estimate the performance, and then aggregate over all items in a training dataset. We give the details in Algorithm \ref{alg:ScaleLaw:Estimation}. 
%\james{Some of the notations below are not consistent with above (e.g. $F_x(t)$) and can be simplified}
}

\begin{algorithm}
\caption{Scaling Law Estimation}\label{alg:ScaleLaw:Estimation}
\KwIn{A training dataset $D_{Tr}=\{x_i, y_i, \{z_{i,m}\}_{k=1}^{K},\{F(t;\{x_i\})\}_{t\in T}^{}\}_{i=1}^{n}$ }
\KwOut{The scaling function $G(K)$}
\For{$i=1$ \KwTo $n$}{
    
    $\hat{y}_i = \arg\max_{a\in A} \sum_{m=1}^{M}\mathbbm{1}_{z_{i,j} = a} $ \tcp{Identify majority choices}
    $G_i(K;\alpha) = \begin{cases}
    g_0(K;\alpha), & \textit{$ y_i = \hat{y}_i $ } \\
        g_1(K;\alpha), & o/w        
    \end{cases}$\tcp{choose the parametric form}

    Obtain $\pmb c_i = \arg\min_{\alpha} \sum_{t\in T}^{} \ell(G_i(t;\alpha), F(t;\{x_i\}))$ \tcp{fit the parameter}
    
}
Return $G(K;D_{Tr}) = \frac{1}{n}\sum_{i =1}^{n} G_i(K;\pmb c_i)$ \tcp{aggregate}
\end{algorithm}

\subsection{Optimization By Filtering}
Next, we study another approach to optimize the one layer system. That is, we add a filtering layer. 




\paragraph{How to model the filtering approach.}
For any fixed query $x$, we quantify the performance of a filter by (i) the probability that an answer is kept given that it is sampled from the correct answer set, denoted by $\alpha$, and (ii) the probability that an answer is kept given that it is sampled from the incorrect answer set, denoted by $\beta$. 
More formally, 

\begin{equation*}
    \alpha=\Pr[z \in h(z) |z  \textit{ is correct}]
\end{equation*}
and 
\begin{equation*}
    \beta=\Pr[z \in h(z) |z  \textit{ is incorrect}]
\end{equation*}

Focusing on a binary case, we have 
$\Pr[\hat{y}=a^*]= \Pr[\sum_{i}^{K} q_i>0] $
where $q_i = xxx $.

\paragraph{When is a query easy or hard?} For voting system, a query is easy iff $r-\frac{1}{2}>0$, where $r=\Pr[z_k=a^*]$ is the correct answer rate.
 For filtering system, a query is easy iff $r \alpha - \frac{1}{2} \beta >0$, where $\alpha=\Pr[\Phi(x,z)=1| z \textit{ is correct} ]$ and $\beta=\Pr[\Phi(x,z)=1]$.



Analyzing the filtering system: Given a user query $x$, we are interested in the probability of the answer produced by the filtering system to be correct, i.e.,
\begin{equation*}
    \Pr[\hat{y}=a^*] = \Pr[\arg\max_{a\in A} \sum_{k=1}^{K}\mathbbm{1}_{z_k=a} w_k = a^*]
\end{equation*}
W.L.O.G, let us assume $a^*=a_1$. Then we have
\begin{equation*}
\arg\max_{a\in A} \sum_{k=1}^{K}\mathbbm{1}_{z_k=a} w_k = a^* \Longleftrightarrow \sum_{k=1}^{K}\mathbbm{1}_{z_k=a_1} w_k > \sum_{k=1}^{K}\mathbbm{1}_{z_k=a_2} w_k
\end{equation*}
Now, noting that $\mathbbm{1}_{z_k=a_2}=1- \mathbbm{1}_{z_k=a_1}$, we have 
\begin{equation*} \sum_{k=1}^{K}\mathbbm{1}_{z_k=a_1} w_k > \sum_{k=1}^{K}\mathbbm{1}_{z_k=a_2} w_k \Longleftrightarrow \sum_{k=1}^{K}\mathbbm{1}_{z_k=a_1} w_k - \frac{1}{2} w_k > 0
\end{equation*}
Therefore, we have 
\begin{equation*}
    \Pr[\hat{y}=a^*] = \Pr[\sum_{k=1}^{K}\mathbbm{1}_{z_k=a_1} w_k - \frac{1}{2} w_k > 0]
\end{equation*}
Note that all terms within the summation are i.i.d. Therefore, $\lim_{K\rightarrow+\infty} \Pr[\hat{y}=a^*]=1$ iff 
\begin{equation*}
\mathbbm{E}[\sum_{k=1}^{K}\mathbbm{1}_{z_k=a_1} w_k - \frac{1}{2} w_k] > 0
\end{equation*}
That is, $r\alpha -\frac{1}{2}\beta>0$.

\paragraph{When the filtering approach is better than voting?}
\begin{theorem}
    The filtering approach is better than the voting approach if and only if $\alpha>\beta$.
\end{theorem}






Now we analyze Voting \LMNets{} with a focus on their scaling properties. In particular, we (i) characterize how \dataitem{}  difficulty shapes the performance landscape, (ii) derive the optimal number of LM calls as a function of the \dataitem{}  difficulty,  
(iii) propose a scaling law, and (iv) present an algorithmic paradigm to estimate the scaling law parameters using a small number of samples. For ease of reference, we have listed all major notations in Table \ref{tab:ScaleLaw:Notations}.



\subsection{Item  Difficulty}
How can we quantify the difficulty of a query item $x$ in an evaluation task? One natural option is  \textit{correct answer rate}, i.e., how likely a candidate answer is correct,  denoted by $r(x) \triangleq \mathbb{E}_{\theta \sim \Theta} [G(x,\theta) =y]\in [0,1]$.
Intuitively, large $r(x)$ indicates that the query $x$ is relatively easy to answer, and small $r(x)$ implies that it is hard. If $r(x)>0.5$, we call  $x$ an ``easy'' query. Otherwise, we call it a ``hard'' query.

Now, we can quantify the difficulty of a data distribution $D$ by a distribution over the item difficulty, denoted by $\mathcal{P}$. That is, for an item $x$ randomly drawn from  $D$, its difficulty $r(x)$ follows   $\mathcal{P}$.

{\color{red} TODO. }

\subsection{Problem Statement}
Our goal is to study the \textit{scaling properties of one-layer Voting \LMNets{}}, i.e., how the number of LM calls $K$ affects an \LMNet{}'s performance on a data distribution $D$, denoted by $F(K;D)$. For exposure purposes, we focus on the expected $0/1$ loss as the performance metric, i.e.,
$F(K;D) = \mathbbm{E}[\hat{y}=y]$, where the expectation is taken over the data distribution $D$ and the sample parameters $\theta_1,\theta_2, \cdots, \theta_K$ in the Voting \LMNet{}. 
Note that our analysis can generalize to other loss functions as well. For simplicity, let us also assume that the difficulty of items in $D$ takes values from only two values. More specifically, for a query $x\in D$,
\begin{align*}
r(x) = \begin{cases}
    p_1, & \textit{ with probability } \alpha \\
    p_2, & \textit{ with probability } 1-\alpha \\
\end{cases}    
\end{align*}
We say that such a $D$ is \textit{$2$-level difficult} with parameter $(\alpha, p_1, p_2)$. W.L.O.G, let us assume $p_1> p_2$.  We also suppose that the answer space $A$ contains only two possible answers.
We will discuss how some of our results can be generalized to the generic difficulty distribution and answer space, but we leave an in-depth as future work.


\subsection{\Dataitem{}  Difficulty Shapes Performance Landscape}
\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figure/method/InferenceNetwork_shape.pdf}
    \caption{How the \dataitem{} difficulties shape the landscape of a one-layer Voting \LMNet{}'s performance. Informally, if the overall task is ``easy'' ($p_1+p_2>1$), but the fraction of ``hard'' queries is large ($\alpha<1-\frac{1}{t}$), then as the number of LM calls increases, the Voting \LMNets{}' performance increases first but then decreases. We call such a landscape a ``inverse U shape''. 
Similarly,  if the overall task is ``hard'' ($p_1+p_2<1$), but the fraction of ``hard'' queries is small ($\alpha>1-\frac{1}{t}$), then enlarging the number of LM calls leads an initial decrease and then increase. Such a landscape is called a ``U shape''. When $\alpha$ is large, the U-shape is less likely to occur while the inverse U-shape becomes more common. Smaller $\alpha$ leads to an opposite trend.}
    \label{fig:ScaleLaw:Landscape}
\end{figure}
How does the \dataitem{} difficulty affect the performance landscape of a one-layer Voting \LMNet{}? The following theorem gives a qualitative characterization. %how the difficulty parameters $(\alpha, p_1, p_2)$ affect the performance landscape. 
 %To answer this, let us first connect \LMNet{}'s performance with data difficulty via the lens of incomplete beta function. 

%Here, the two terms correspond to the performance on queries with difficulty $p_1$ and $p_2$ respectively. It is easy to see that the performance is monotonically increasing (or decreasing) if both $p_1,p_2$ are larger (or smaller) than $\frac{1}{2}$. It becomes interesting when $p_1>\frac{1}{2}$ and $p_2<\frac{1}{2}$: as $K$ increases, the first incomplete beta function becomes larger, but the second incomplete beta function gets smaller. The following theorem qualitatively characterizes how the difficulty parameters $(\alpha, p_1, p_2)$ affect the performance landscape. 

%\james{If there are three or more levels of difficulty, can the curve have multiple ups and downs?}

\begin{theorem}\label{thm:scaleLaw:character}
Suppose $D$ is $2$-level difficult with $(\alpha, p_1,p_2)$,  $\|A\|=2$, and $K$ is odd W.L.O.G. Let $t\triangleq \frac{p_2 (1-p_2) (\frac{1}{2}-p_2)}{p_1 (1-p_1) (p_1-\frac{1}{2})}+1$. If  $p_1+p_2\not=1$ and $p_2<\frac{1}{2}<p_1$, then as $K$ increases, $F(K;D)$ 
   \begin{itemize}
       \item  increases monotonically, if $p_1+p_2>1$ and  $\alpha \geq 1-\frac{1}{t}$
       \item decreases monotonically,  if $p_1+p_2<1$ or $\alpha\leq 1-\frac{1}{t}$
       \item increases and then decreases, if $p_1+p_2>1$ and $\alpha<1-\frac{1}{t}$
       \item decreases and then increases, if $p_1+p_2<1$ and $\alpha>1-\frac{1}{t}$
   \end{itemize}
   \end{theorem}

Theorem \ref{thm:scaleLaw:character} precisely connects the \dataitem{} difficulty with the performance landscape. Here, $t$ is a constant that only depends on $p_1$ and $p_2$, i.e., the probability of an LM's generation being correct on easy and hard queries, respectively. Intuitively, $t$ quantifies the difficulty similarity between the easy and hard queries: it becomes larger if the easy queries are more difficult ($p_1$ is smaller) or the hard queries are less difficult ($p_2$ is larger).  Interestingly, it suggests that, for some \dataitem{} difficulty distribution, a non-monotone effect of the number of LM calls is expected. Informally, if the overall task is ``easy'' ($p_1+p_2>1$), but the fraction of ``hard'' queries is large ($\alpha<1-\frac{1}{t}$), then as the number of LM calls increases, the Voting \LMNets{}' performance increases first but then decreases. We call such a landscape a ``inverse U shape''. 
Similarly,  if the overall task is ``hard'' ($p_1+p_2<1$), but the fraction of ``hard'' queries is small ($\alpha>1-\frac{1}{t}$), then enlarging the number of LM calls leads an initial decrease and then increase. Such a landscape is called a ``U shape''. 
This well explains the U-shape of \LMNets{}' performance shown in Figure \ref{fig:ScaleLaw:intro1}.Figure \ref{fig:ScaleLaw:Landscape} visualizes the effects of \dataitem{} difficulty on the performance landscape in more detail. 

\subsection{\Dataitem{} Difficulty Determines Optimal Number of LM Calls}
We have shown that there are cases where, determined by \dataitem{} difficulty distribution,   a non-monotone scaling behavior of Voting \LMNets{} is expected.  In these cases, blindly scaling up the number of LM calls may not lead to the desired performance. 
How should one determine the number of LM calls in these cases? The following result gives a precise answer.

\begin{theorem}\label{thm:scalelaw:optimalnetworksize}
Suppose $D$ is $2$-level difficult with $(\alpha, p_1,p_2)$, $\|A\|=2$, and $K$ is odd W.L.O.G. If $p_1+p_2>1$ and $\alpha<1-\frac{1}{t}$, then the number of LM calls  $K^*$ that maximizes the overall performance of an one-layer Voting \LMNet{}(up to rounding) is 
\begin{align*}
    K^* = 2 \frac{\log\frac{\alpha}{1-\alpha}\frac{2p_1-1}{1-2p_2}}{\log \frac{p_2(1-p_2)}{p_1(1-p_1)}} 
\end{align*}
\end{theorem}
As expected, the optimal number of LM calls depends on the \dataitem{} difficulty. For example, $K^*$ will be larger if $\alpha$ grows (up to $1-\frac{1}{t}$). 
That is, if there are more ``easy'' queries than ``hard'' queries, then a larger network should be adopted. This suggests that a difficulty-aware design of Voting \LMNets{} may offer better performance than a difficulty-agnostic design. We will analyze $K^*$ in detail in Section \ref{sec:scalelaw:exp_optimalsize}. 


\subsection{A Scaling Law for One-layer Voting \LMNets{}}
We have seen that inference system performance is closely related to item difficulty. 
What is an intuitive way to explicitly model \dataitem{} difficulty in a scaling law of Voting \LMNets{}? 
Here, we propose the following function $G(\cdot;\cdot)$ 
 as a scaling law on the dataset $D$ with 2-level difficulty 
\begin{align*}
G(K;D) \triangleq \alpha g_{p_1}(K;\pmb c_1) + (1-\alpha) g_{p_2}(K;\pmb c_2)   
\end{align*}
where 
\begin{align*}
    g_p(K;\pmb c) \triangleq \begin{cases}
       1 - \exp(- \pmb c^T [K,\sqrt{K},1]) & \textit{if } p> \frac{1}{2}\\
       \exp(- \pmb c^T [K,\sqrt{K},1])  &  \textit{if } p< \frac{1}{2} \\
    \end{cases}
\end{align*}
This scaling law encodes how the \dataitem{} difficulty affects the performance. For example, if  $p_1>\frac{1}{2}$ and $p_2<\frac{1}{2}$, the first term $g_{p_1}(\cdot;\cdot)$ will monotonically increase while the second term $g_{p_2}(\cdot;\cdot)$ will  monotonically decrease, and hence the overall scaling function $G(K;D)$ exhibits a non-monotone behavior. This also captures that the number of LM calls changes the performance at an exponential rate.

This scaling law can be easily generalized to data $D$ with generic \dataitem{} difficulty distribution. In particular, if the density function of the \dataitem{} difficulty is $q(u)$, then we can generalize the scaling law for the 2-level difficulty to this case via 
\begin{align*}
G(K;D) \triangleq \int_{0}^{1}  g_{q(u)}(K;\pmb c_u) q(u) d u     
\end{align*}
For discrete distribution, one can simply replace the integral by summation and the density function by the mass function.

\subsection{Estimating the Scaling Law Parameters}
In practice, an important problem is to learn the scaling law using a small number of samples. Here, we give an algorithmic paradigm to estimate the scaling law parameters and thus the overall scaling function $G(\cdot;\cdot)$, as shown in Algorithm \ref{alg:ScaleLaw:Estimation}.

The estimation paradigm contains two major steps: it first estimates the scaling parameter for each item in the training dataset, and then aggregates the results to obtain the overall scaling function. To estimate the scaling law on each item, it first compares the majority vote on a few samples (line 2) with the true label to determine if the query is easy or not and thus selects the parametric form (line 3). Then it uses the empirically observed performance on a few samples to fit the parameters (line 4). For demonstration purposes, we use a square loss function as the optimization metric. %\james{explain what loss function we use for estimation in step 4.}. 
Finally, the aggregation (line 5) over each item's scaling function is returned as the final estimation.


\eat{\paragraph{Generalization to generic data distribution.} By definition, the performance on a generic data with difficulty distribution $\mathcal{P}$ is $F(K;D) = \mathbbm{E} [y=\hat{y}] = \mathbbm{E}[\mathbbm{E}[y=\hat{y}|r(x)=p] \cdot \mathbbm{1}_{r(x)=p}] = \mathbbm{E}[ I_p(\frac{K+1}{2},\frac{K+1}{2}) \cdot \mathbbm{1}_{r(x)=p}]$. Let $p(\cdot)$ denote the pdf (or pmf) of $r(x)$. We can rewrite this as  $F(K;D) = \int_{0}^{1} I_t(\frac{K+1}{2},\frac{K+1}{2}) p(t) dt$. It is challenging to precisely characterize how the difficulty distribution $\mathcal{P}$ affects the performance landscape and optimal network sizes due to the integral. However, one can still show that there exists some difficulty distribution $\mathcal{P}$, such that the shape of the performance landscape can be monotone, a U-shape, or even zig-zag. This further highlights the importance of carefully choosing the network sizes. 

\paragraph{Generalization to tasks with answer space size $\|A\|>2$.} A precise analysis for generic tasks is even more challenging, as there is no closed form for the performance on an individual item with difficulty $p$. Fortunately, we can give an upper and lower bound on it. To see this, simply note, among all candidate answers, (i) that if the fraction of correct answers is larger than $\frac{1}{2}$, then the correct answer must be choices of majority vote, and (ii) that if the correct answer is the majority vote, then at least $\frac{1}{\|A\|}$ fraction of answers must be correct. This gives the inequality 
$
\Pr\left[\frac{1}{K}\sum^{K}_{i=1}\mathbbm{1}_{z_i =y}> \frac{1}{d}\right]   \geq  \mathbbm{E}[{y=\hat{y}}] \geq  \Pr\left[\frac{1}{K}\sum^{K}_{i=1}\mathbbm{1}_[z_i=y] > \frac{1}{2}\right]
$. Thus, aggregating both sizes over the difficulty distributions gives an upper and lower bound on the overall performance on a generic distribution $D$ with arbitrary answer space size.

What does the above analysis imply in practice? One important observation is that we can predict \LMNet{} performance on generic data with arbitrary answer space. To see this, notice that the upper and lower bounds can both be approximated by the function $g(K;a_1, a_2, a_3)$ with varying parameters $a_1, a_2, a_3$. Thus, for each item, we can directly fit $a_1, a_2, a_3$ to estimate the performance, and then aggregate over all items in a training dataset. We give the details in Algorithm \ref{alg:ScaleLaw:Estimation}. 
%\james{Some of the notations below are not consistent with above (e.g. $F_x(t)$) and can be simplified}
}

\begin{algorithm}
\caption{Scaling Law Estimation}\label{alg:ScaleLaw:Estimation}
\KwIn{A training dataset $D_{Tr}=\{x_i, y_i, \{z_{i,m}\}_{k=1}^{K},\{F(t;\{x_i\})\}_{t\in T}^{}\}_{i=1}^{n}$ }
\KwOut{The scaling function $G(K)$}
\For{$i=1$ \KwTo $n$}{
    
    $\hat{y}_i = \arg\max_{a\in A} \sum_{m=1}^{M}\mathbbm{1}_{z_{i,j} = a} $ \tcp{Identify majority choices}
    $G_i(K;\alpha) = \begin{cases}
    g_0(K;\alpha), & \textit{$ y_i = \hat{y}_i $ } \\
        g_1(K;\alpha), & o/w        
    \end{cases}$\tcp{choose the parametric form}

    Obtain $\pmb c_i = \arg\min_{\alpha} \sum_{t\in T}^{} \ell(G_i(t;\alpha), F(t;\{x_i\}))$ \tcp{fit the parameter}
    
}
Return $G(K;D_{Tr}) = \frac{1}{n}\sum_{i =1}^{n} G_i(K;\pmb c_i)$ \tcp{aggregate}
\end{algorithm}

\subsection{Optimization By Filtering}
Next, we study another approach to optimize the one layer system. That is, we add a filtering layer. 




\paragraph{How to model the filtering approach.}
For any fixed query $x$, we quantify the performance of a filter by (i) the probability that an answer is kept given that it is sampled from the correct answer set, denoted by $\alpha$, and (ii) the probability that an answer is kept given that it is sampled from the incorrect answer set, denoted by $\beta$. 
More formally, 

\begin{equation*}
    \alpha=\Pr[z \in h(z) |z  \textit{ is correct}]
\end{equation*}
and 
\begin{equation*}
    \beta=\Pr[z \in h(z) |z  \textit{ is incorrect}]
\end{equation*}

Focusing on a binary case, we have 
$\Pr[\hat{y}=a^*]= \Pr[\sum_{i}^{K} q_i>0] $
where $q_i = xxx $.

\paragraph{When is a query easy or hard?} For voting system, a query is easy iff $r-\frac{1}{2}>0$, where $r=\Pr[z_k=a^*]$ is the correct answer rate.
 For filtering system, a query is easy iff $r \alpha - \frac{1}{2} \beta >0$, where $\alpha=\Pr[\Phi(x,z)=1| z \textit{ is correct} ]$ and $\beta=\Pr[\Phi(x,z)=1]$.



Analyzing the filtering system: Given a user query $x$, we are interested in the probability of the answer produced by the filtering system to be correct, i.e.,
\begin{equation*}
    \Pr[\hat{y}=a^*] = \Pr[\arg\max_{a\in A} \sum_{k=1}^{K}\mathbbm{1}_{z_k=a} w_k = a^*]
\end{equation*}
W.L.O.G, let us assume $a^*=a_1$. Then we have
\begin{equation*}
\arg\max_{a\in A} \sum_{k=1}^{K}\mathbbm{1}_{z_k=a} w_k = a^* \Longleftrightarrow \sum_{k=1}^{K}\mathbbm{1}_{z_k=a_1} w_k > \sum_{k=1}^{K}\mathbbm{1}_{z_k=a_2} w_k
\end{equation*}
Now, noting that $\mathbbm{1}_{z_k=a_2}=1- \mathbbm{1}_{z_k=a_1}$, we have 
\begin{equation*} \sum_{k=1}^{K}\mathbbm{1}_{z_k=a_1} w_k > \sum_{k=1}^{K}\mathbbm{1}_{z_k=a_2} w_k \Longleftrightarrow \sum_{k=1}^{K}\mathbbm{1}_{z_k=a_1} w_k - \frac{1}{2} w_k > 0
\end{equation*}
Therefore, we have 
\begin{equation*}
    \Pr[\hat{y}=a^*] = \Pr[\sum_{k=1}^{K}\mathbbm{1}_{z_k=a_1} w_k - \frac{1}{2} w_k > 0]
\end{equation*}
Note that all terms within the summation are i.i.d. Therefore, $\lim_{K\rightarrow+\infty} \Pr[\hat{y}=a^*]=1$ iff 
\begin{equation*}
\mathbbm{E}[\sum_{k=1}^{K}\mathbbm{1}_{z_k=a_1} w_k - \frac{1}{2} w_k] > 0
\end{equation*}
That is, $r\alpha -\frac{1}{2}\beta>0$.

\paragraph{When the filtering approach is better than voting?}
\begin{theorem}
    The filtering approach is better than the voting approach if and only if $\alpha>\beta$.
\end{theorem}


